SGD: The Role of Implicit Regularization, Batch-size and Multiple-epochs

Multi-epoch, small-batch, Stochastic Gradient Descent (SGD) has been the method of choice for learning with large over-parameterized models. A popular theory for explaining why SGD works well in practice is that the algorithm has an implicit regularization that biases its output towards a good solution. Perhaps the theoretically most well understood learning setting for SGD is that of Stochastic Convex Optimization (SCO), where it is well known that SGD learns at a rate of $O(1/\sqrt{n})$, where $n$ is the number of samples. In this paper, we consider the problem of SCO and explore the role of implicit regularization, batch size and multiple epochs for SGD. Our main contributions are threefold: (a) We show that for any regularizer, there is an SCO problem for which Regularized Empirical Risk Minimzation fails to learn. This automatically rules out any implicit regularization based explanation for the success of SGD. (b) We provide a separation between SGD and learning via Gradient Descent on empirical loss (GD) in terms of sample complexity. We show that there is an SCO problem such that GD with any step size and number of iterations can only learn at a suboptimal rate: at least $\widetilde{\Omega}(1/n^{5/12})$. (c) We present a multi-epoch variant of SGD commonly used in practice. We prove that this algorithm is at least as good as single pass SGD in the worst case. However, for certain SCO problems, taking multiple passes over the dataset can significantly outperform single pass SGD. We extend our results to the general learning setting by showing a problem which is learnable for any data distribution, and for this problem, SGD is strictly better than RERM for any regularization function. We conclude by discussing the implications of our results for deep learning, and show a separation between SGD and ERM for two layer diagonal neural networks.

==> files/GD_kink_lb_proof.tex <==
%!TEX root=../paper.tex
In the following, we provide a learning setting for which GD run with step size $\eta < 1/64 n^{5/4}$ has lower bound of $\Omega(1/n^{3/8})$. 
 
\begin{lemma}
\label{lem:small_step_size_lb}
 Let $w \in \bbR$ denote the optimization variable, and $z$ denote a data sample. There exists a function $f(w; z)$ and a distribution $\cD$ over $z$ such that: 
\begin{enumerate}[label=(\alph*), leftmargin=8mm]  
\item The population loss $F(w) \ldef{} \En_{z \sim \cD} \brk*{f(w; z)}$ is $1$-Lipschitz and convex in $w$. Furthermore, there exists a point $w^* \in \argmin_{w} F(w)$ such that $\nrm*{w^*} = 1$. 
\item The variance of the gradient is bounded, i.e. $\En_{z \sim \cD} \brk{\nrm*{\grad f(w; z) - \grad F(w)}^2} \leq 1$ for any $w \in \bbR$. 
\item If $\eta < 1/ 64 n^{5/4}$, then for any $T > 0$, the point $\wgd_T$ returned by running GD algorithm with step size $\eta$ for $T$ steps satisfies 
\begin{align*} 
	\En \brk{ F({{\widehat{w}}^{\text{GD}}}_T)} - \min_{w \in \bbR} F(w) = \Omega\prn[\Big]{\frac{1}{n^{3/8}}}. \numberthis \label{eq:SGD_upper_bound_fn} 
\end{align*}  
\end{enumerate} 
\end{lemma} 
\begin{proof} Before delving into the construction of the function $f$, we first define some  auxiliary functions and  notation. Define the kink function $h(w)$ as 
\begin{align*} 
h(w) \ldef{} \begin{cases} 0 & \text{if} \quad w < 0 \\   
- n^{5/8} w & \text{if} \quad  0 \leq w < \frac{1}{64 n^{5/4}} \\  
~~~ n^{5/8} w - \frac{2}{64 n^{5/8}} & \text{if} \quad \frac{1}{ 64 n^{5/4}} \leq w \leq \frac{3}{ 64 n^{5/4}} \\  
- n^{5/8} w + \frac{4}{64 n^{5/8}}  & \text{if} \quad \frac{3}{64 n^{5/4}} < w   \leq \frac{1}{16 n^{5/4}} \\ 
0 & \text{if} \quad \frac{1}{16 n^{5/4}} \leq w 
\end{cases},  \numberthis \label{eq:kink_definition} 
\end{align*} and the corresponding gradients $\grad h(w)$ as 
\begin{align*}
\grad h(w) \ldef{} \begin{cases} 0 & \text{if} \quad w < 0 \\ 
- n^{5/8} & \text{if} \quad  0 \leq w < \frac{1}{64 n^{5/4}} \\  
n^{5/8}& \text{if} \quad \frac{1}{ 64 n^{5/4}} \leq w \leq \frac{3}{ 64 n^{5/4}} \\ 
- n^{5/8}  & \text{if} \quad \frac{3}{64 n^{5/4}} < w   \leq \frac{1}{16 n^{5/4}} \\ 
0 & \text{if} \quad \frac{1}{16 n^{5/4}} \leq w  
\end{cases}.  \numberthis \label{eq:kink_grad_definition} 
\end{align*} 

Additionally, define the set 
\begin{align*}
H \ldef{} \crl*{\frac{1}{4} + \frac{1}{8 n^{5/4}},   \frac{1}{4} + \frac{2}{8 n^{5/4}}, \ldots, \frac{3}{4}}, 
\end{align*}
where the set $H$ has $4 n^{5/4}$ numbers from the interval $[1/4, 3/4]$ spaced at a distance of $1 / 8n^{5/4}$. 

We now present our learning setting:  
\begin{enumerate}[label=$\bullet$, leftmargin=8mm] 
\item \textit{Data sample:} $z$ consists of the tuple $(\beta, y)$ where $\beta \in H$ and $y \in \crl{-1, +1}$. 

\item \textit{Data Distribution:} $\cD$ over the instances $z = (\beta, y)$ is defined such that 
\begin{align*} 
	\beta \sim \text{Uniform}(H) \qquad \text{and} \qquad y \sim \text{Uniform}(\crl{-1, 1}),  \numberthis \label{eq:step_lb_dist} 
\end{align*} where $\beta$ and $y$ are sampled independent of each other. 

\item \textit{Loss function:} is defined as 
\begin{align*}
	f(w; z) &\ldef{} \frac{1}{n^{3/8}} \max\crl*{-w, -1} + y \cdot {h(w + \beta)},  \numberthis \label{eq:step_lb_func} 
\end{align*} 

Additionally, define the population loss $F(w) \ldef{} \En_{z \sim \cD} \brk*{f(w; z)}$. 
\end{enumerate} 

We next show the desired statements for this learning setting: 
\begin{enumerate}[label=$(\alph*)$, leftmargin=8mm]  
\item For the distribution $\cD$ defined in \pref{eq:step_lb_dist}, since $\En \brk*{y} = 0$ and $y$ is sampled independent of $\beta$, we have that the population loss  
\begin{align*} 
F(w) = \En_{z \sim \cD} \brk*{f(w; z)} = \frac{1}{n^{3/8}} \max \crl{-w, -1}.  
\end{align*} 

Clearly, $F(w)$ is $1$-Lipschitz and convex is $w$. Additionally, the point $w^* = 1$ is a minimizer of $F(w)$. 

\item We next bound variance of the stochastic gradient. For any $w \in \bbR$, we have 
\begin{align*}
\En_{z \sim \cD} \brk{\abs*{\grad f(w; z) - \grad F(w)}^2} &= \En_{(\beta, y)} \brk*{ \abs{ y \grad h(w + \beta) }^2} \\ 
&= \En_{\beta} \brk*{ \abs{ \grad h(w + \beta) }^2}  \\ 
&=  \En_{\beta} \brk[\Big]{ \indic\crl[\Big]{\beta \in \brk[\big]{w - \frac{1}{16 n^{5/4}}, w}} \cdot n^{5/4}} \\ 
&= n^{5/4} \Pr \prn[\big]{\beta \in \brk[\big]{w - \frac{1}{16 n^{5/4}}, w}}  
\end{align*} where the equality in the first line holds because $y \in \crl*{-1, 1}$, and the second line follows from the construction of the function $h$ which implies that $\abs{\grad h(w + \beta)} \leq n^{5/8}$ for any $w$ and $\beta$ (see \pref{eq:kink_grad_definition}). Using the fact that $\beta \sim \text{Uniform}(B)$ in the above, we get that  
\begin{align*} 
\En_{z \sim \cD} \brk{\abs*{\grad f(w; z) - \grad F(w)}^2} &\leq 1/4. 
\end{align*} 

\item We next show that GD algorithm when run with the step size of $\eta \leq 1/ 64 n^{5/4}$ fails to converge to a good solution. 

Define $\beta_{(1)}, \ldots, \beta_{(n)}$ such that $\beta_{(j)}$ denotes the $j$th smallest item in the set $\crl*{\beta_1, \ldots, \beta_n}$, and define $y_{(j)}$ as the corresponding $y$ variable for the random variable $\beta_{(j)}$. An application of \pref{lem:technical_lemma_4} implies that with probability at least $1 - 2 / n^{1/4}$, there exists a $\wh j \leq \ceil{{\log(n)}/{2 n ^{1/4}}}$ such that: 
\begin{enumerate}[label=$(\alph*)$, leftmargin=8mm]
\item[$\proman{1}$] $\beta_{(1)} \neq \beta_{(2)} \neq \beta_{(3)} \neq \cdots \neq \beta_{(\wh j + 1)}$, and 
\item[$\proman{2}$] $y_{(\wh j)} = +1$. 
\end{enumerate} 

In the following, we condition on the occurrence of the above two events. The key idea of the proof is that at the level of the empirical loss, the first $\wh j$ kinks (that arise as a result of the stochastic function $h$) would be isolated from each other due to event-$\proman{1}$. Thus, the norm of the gradient of the empirical loss would be bounded by $2 / n^{3/8}$ for all points before $\beta_{\wh j}$. At the same time, since $y_{(\wh j)} = +1$ from event-$\proman{2}$, the empirical loss would be flat in a small interval around $\beta_{\wh j}$. As we show in the following, when GD is run on the empirical loss with step size $\eta \leq 1/64 n^{5/4}$, some GD iterate will lie in this small flat region, and after that GD will fail to make progress because the gradient is $0$; hence outputting a bad solution. On the other hand, GD / SGD run with a large step size e.g. $1/\sqrt{n}$ will easily jump over these kinks and converge to a good solution. We illustrate this intuition in \pref{fig:emp_loss}, and provide the proof below. 

\begin{figure}[ht]
\begin{flushright}
{\includegraphics[width=1.1\textwidth]{files/emp_loss}}
\end{flushright}
\caption{(Picture not drawn according to scale) The solid red line shows the empirical loss induced by the kink function when $y = +1$, the solid green line shows the empirical loss when $y = -1$, and the dotted blue line shows the convex population loss. The empirical loss when $y = +1$ has gradient $0$ in a region of width $1/32 n^{5/4}$. Gradient descent with step size smaller than $1/64 n^{5/4}$, shown in the bottom, will get stuck in this flat region and thus fail to find a good solution. On the other hand, gradient descent with large step size will jump over the kink and find a good solution.} 
\label{fig:emp_loss}  	
\end{figure} 

Recall that the empirical loss on the dataset $S$ is given by: 
\begin{align*} 
	\wh F(w) = \frac{1}{n^{3/8}} \max \crl{-w, -1} + \frac{1}{n} \sum_{j=1}^n y_{j} \prn*{h(w + \beta_j)} 
\end{align*} 
Note that for any $\beta \in H$, the set of $w$ for which $h(w + \beta)$ is non-zeros is given by the interval $[\beta, \beta + 1/16n^{5/4}]$. Furthermore, any two numbers in the set $H$ are at least $1/8n^{5/4}$ apart from each other. Thus, the event-$\proman{1}$ above implies that non-zero parts of the functions $\crl{h(w + \beta_{(1)}), \ldots, h(w + \beta_{(\wh j)})}$, i.e. the first $\wh j$ kinks do not overlap with each other. This implies that for $w <  \beta_{(\wh j + 1)}$, 
\begin{align*}
\abs{\grad \wh F(w)} &\leq \frac{1}{n^{3/8}} + \frac{1}{n} \sum_{j=1}^n \abs{\grad {h(w + \beta_j)}} \\ &\leq \frac{1}{n^{3/8}} + \frac{n^{5/8}}{n} \leq \frac{2}{n^{3/8}},  \numberthis \label{eq:gradient_lipschitz}  
\end{align*}
where the first inequality in the above follows from Triangle inequality and the second inequality holds because at most one of the $n$ terms in the stochastic component $\sum_{j=1}^n y_{j} \prn*{h(w + \beta_j)}$ above is non-zero for $w <  \beta_{(\wh j + 1)}$. Thus, $\wh F(w)$ is $1$-Lipschitz for $w \in [0, \beta_{(\wh j + 1)})$. 

Next, the event-$\proman{2}$ above implies that $y_{(\wh j)} = 1$. Define the interval $\wt \cW \ldef{} (\beta_{(\wh j)} + 1/64 n^{5/4}, \beta_{(\wh j)} + 3/64 n^{5/4})$ and note that for any $w \in \wt \cW$, 
\begin{align*}
\grad \wh F(w) &= - \frac{1}{n^{3/8}} + \frac{1}{n} \grad h(w + \beta_{(\wh j)}) \\ 
 &= - \frac{1}{n^{3/8}}  + \frac{1}{n} \cdot n^{5/8} = 0,  \numberthis \label{eq:gradient_flat} 
\end{align*} where the first equality holds because $y_{(\wh j)} = +1$ and using the event-$\proman{1}$ above. This implies that the empirical loss $\wh F(w)$ has $0$ gradient for $w \in \wt \cW$, and thus GD algorithm will stop updating if any iterate reaches $\wt \cW$. 


In the following, we will show that for $\eta \leq 1/ 64 n^{5/4}$, GD algorithm is bound to get stuck in the interval $\wt \cW$, and will thus fail to find a good solution. Consider the dynamics of the GD algorithm:
\begin{align*} 
w_{t + 1} \leftarrow w_{t} - \eta \grad \wh F(w_{t}), 
\end{align*} 
where the initial point  $w_1 = 0$. Suppose there exists some time $\tau$ for which  $w_{\tau} > \beta_{(\wh j + 1)}$, and let $t_0 > 0$ denote the smallest such time. Thus, for any $t < t_0$ and $\eta \leq 1/64 n^{5/4}$, we have that 
\begin{align*}
\abs{w_{t + 1} - w_{t}} &= \eta \abs{ \grad \wh F(w)} \leq \eta \leq 1/64 n^{5/4}, 
\end{align*}
where the first inequality holds due to \pref{eq:gradient_lipschitz}.  This implies that any two consecutive iterates produced by the GD algorithm for $t < t_0$ are at most $1/64 n^{5/4}$ apart from each other. However, note that the interval $\wt \cW  \subseteq  [0, \beta_{(\wh j + 1)})$ and has width of $2/64 n^{5/4}$. Thus, there exists some time $t' \leq t_0$ for which $w_{t'}$ will lie in the set $\wt \cW$. However, recall that $\grad F(w) = 0$ for any $w \in \wt \cW$ as shown in \pref{eq:gradient_flat}. Thus, once $w_{t'} \in \wt \cW$, GD will not update any further implying that for all $t > t'$, $w_{t} = w_{t'}.$ This shows via contradiction that no such time $\tau$ exists for which $w_{\tau} > \beta_{(\wh j + 1)}$. 

Hence for $\eta < 1/64 n^{5/4}$, all iterates $\crl{w_t}_{t \geq 0}$ generated by the GD algorithm will lie in the set $[0, \beta_{(\wh j + 1)})$. Thus, for any $T > 1$, the returned point $\wgd_T$ satisfies
\begin{align*}
\wgd_T \leq \beta_{(\wh j + 1)} \leq \frac{3}{4}, 
\end{align*} where the second inequality holds because $\beta_{(\wh j + 1)} \in H$ and is thus smaller than $3/4$. Thus, 
\begin{align*}
 F({{\widehat{w}}^{\text{GD}}}_T) - \min_{w \in \bbR} F(w) \geq \frac{1}{4 n^{3/8}}. \numberthis \label{eq:lower_bound_flat_final} 
\end{align*}

Since, the events $\proman{1}$ and $\proman{2}$ occur simultaneously with probability at least $1 - 2 / n^{1/4}$, we have that for any $T \geq 0$, 
\begin{align*} 
	\En \brk{ F({{\widehat{w}}^{\text{GD}}}_T)} - \min_{w \in \bbR} F(w) = \Omega\prn[\big]{\frac{1}{n^{3/8}}}. 
\end{align*} 
\end{enumerate} 
\end{proof}

\begin{lemma} 
\label{lem:technical_lemma_4}  
Suppose $(\beta_1, y_1), \ldots, (\beta_n, y_n)$ be $n$ samples drawn independently from $\textit{Uniform}(H) \times \text{Uniform}(\crl{-1, 1})$, where the set 
$H \ldef{} \crl{\tfrac{1}{4} + \tfrac{1}{8 n^{5/4}},   \tfrac{1}{4} + \tfrac{2}{8 n^{5/4}}, \ldots, \tfrac{3}{4}}$. Further, define $\beta_{(j)}$ to denote the $j$th smallest number in the set $\crl*{\beta_1, \ldots, \beta_n}$, and define $y_{(j)}$ as the corresponding $y$ variable for $\beta_{(j)}$. Then, with probability at least $1 - 2 / n^{1/4}$, there exists a $\wh j \leq  \ceil{{\log(n)}/{2 n ^{1/4}}}$ such that: 
\begin{enumerate}[label=$(\alph*)$, leftmargin=8mm]
\item[$\proman{1}$] $\beta_{(1)} \neq \beta_{(2)} \neq \beta_{(3)} \neq \cdots \neq \beta_{(\wh j + 1)}$, and 
\item[$\proman{2}$] $y_{(\wh j)} = +1$. 
\end{enumerate} 
\end{lemma}
\begin{proof} Let $k = \ceil{{\log(n)}/{2 n ^{1/4}}}$. We give the proof by translating our problem into a ``ball and bins" problem. 

Let the set $H$ denote $m = 4 n^{5/4}$ distinct bins, and let there be $n$ distinct balls. Each of the $n$ balls are tossed independently into one of the $m$ bins drawn uniformly at random. For any $i, j$, the event where the ball $j$ is tossed into the bin $i$ corresponds to the event that $\beta_j = \tfrac{1}{4} + \frac{i}{8 n^{5/4}}$. In addition to this, the balls are such that they change color after they are tossed into a bin. In particular, after being tossed into a bin, a ball changes color to either red or blue with equal probability. For any $i, j$, the event where the ball $j$ takes red color corresponds to the event that $y_j = 1$; Similarly, blue color corresponds to $y = -1$. Thus, in the balls and bins model, the position of the $n$ balls in the bins and their corresponding colors after tossing reveals the value of the random variables $(\beta_1, y_1), \ldots, (\beta_n, y_n)$.

In the following, we first show that with probability at least $1 - \frac{2}{n^{1/4}}$, the first $k$ bins will have at most one ball each, and there will be some bin amongst the first $k$ bins that contains a red color ball. Define $E_{i}$ to denote the event that the bin $i$ gets more than one ball. Thus, 
\begin{align*}
	\Pr(E_i) &= 1 - \Pr (\text{Bin $i$ has $0$ or $1$ ball in it}) \\
					&= 1 - \prn[\Big]{1 - \frac{1}{n^{5/4}}}^n -  n \prn[\Big]{1 - \frac{1}{n^{5/4}}}^{n-1} \frac{1}{n^{5/4}} \\ 					
					&\leq  1 - \prn[\Big]{1 - \frac{1}{n^{1/4}}} - \frac{1}{n^{1/4}}\prn[\Big]{1 - \frac{n - 1}{n^{5/4}}} \\
					&= \frac{n - 1}{n^{3/2}} \leq \frac{1}{\sqrt{n}}  \numberthis \label{eq:E_i_bound_bnb}
\end{align*} where the first inequality in the above follows from the fact that $(1- \alpha)^n \leq 1 - \alpha n$ for any $\alpha \geq -1$ and $n \geq 1$. Let $A_k$ denote the event that there exists some bin among the first $k$ bins that has more than one ball. Taking a union bound, we get   
\begin{align*}
\Pr \prn{A_k} = \Pr \prn{\cup_{i=1}^{k} E_i}  &\leq \sum_{i=1}^{k} \Pr \prn*{E_i}  \leq \frac{k}{\sqrt{n}}. 
\end{align*}

Next, let $B_k$ denote the event that there is no red ball in the first $k$ bins after $n$ tosses. When we throw a ball, the probability that it will fall in the first $k$ bins is given by ${k}/{n^{5/4}}$, and the probability that it takes the color red is ${1}/{2}$. Since the bin chosen and the final color are independent of each other for each ball, the probability that a ball falls into the first $k$ bins and is of red color is given by $k/2n^{5/4}$. Furthermore, since the balls are thrown independent to each other, the probability that if we throw $n$ balls, no ball falls into the first $k$ bins that takes the red color is given by 
\begin{align*}
\Pr \prn*{B_k} &= \prn[\Big]{1 - \frac{k}{2 n^{5/4}}}^n. 
\end{align*}

Finally, let us define $C_k$ to denote the event that there is at most one ball per bin amongst the first $k$ bins, and that there exists a bin amongst the first $k$ bins with a red ball in it. By the definition of the events $A_k$ and $B_k$, we note that 
\begin{align*}
\Pr \prn*{C_k} &= \Pr \prn*{A_k^{c} \cap B_k^{c}} \\
						&= 1 - \Pr \prn*{A_k \cup B_k}  \\ 
						  &\geq 1 - \Pr(A_k) - \Pr(B_k) \\ 
						  &\geq 1 - \frac{k}{\sqrt{n}} - \prn[\Big]{1 - \frac{k}{2n ^{5/4}}}^n \\ 
						  &\geq 1 - \frac{k}{\sqrt{n}} - e^{- k/ 2 n^{1/4}}, 
\end{align*} where the first inequality in the above follows from the union bound, the second inequality holds by plugging in the corresponding bounds for $P(A_k)$ and $P(B_k)$, and the last line is due to the fact that $(1 + \alpha)^n \leq e^{\alpha n}$ for any $\alpha$. Plugging in the value of $k = \ceil{{\log(n)}/{2 n ^{1/4}}}$ in the above, we get that 
\begin{align*} 
\Pr \prn*{C_k} &\geq 1 - \frac{2}{n^{1/4}}. 
\end{align*} 
 
Thus, with probability at least $1 - 2 / n^{1/4}$, the first $k$ bins have at most one ball each, and there exists some bin $\wh j \in [k]$ that contains a red ball; when this happens, the corresponding random variables  $(\beta_1, y_1), \ldots, (\beta_n, y_n)$ satisfy: 
\begin{enumerate}[label=$(\alph*)$, leftmargin=8mm] 
\item $\beta_{(1)} \neq \beta_{(2)} \neq \beta_{(3)} \neq \cdots \neq \beta_{(\wh j + 1)}$, and 
\item $y_{(\wh j)} = +1$. 
\end{enumerate} 
\end{proof} 


==> files/app_sgd_vs_gd.tex <==
%!TEX root=../paper.tex 
Throughout this section, we assume that a data sample $z$ consists of $(x, y, \alpha)$, where $x \in \{0,1\}^d$, $y \in \crl{-1, 1}$ and $\alpha \in \{0,e_1,\ldots,e_d\}$, and the loss function $f:\reals^d \times \cZ$ is given by: 
\begin{align} 
  f(\w; (x,y,\alpha)) = y \nrm*{(\w - \alpha) \odot x}. 
\end{align} 
Since $f$ is not differentiable when $w = 0$, we define the sub-gradient $\partial f(\w) = 0$. Furthermore, we will be using the distributions $D(\delta, p, a)$, defined in \pref{def:violating_distribution_defn}. 

\subsection{Proof of \pref{lem:lem1_main_gdvssgd}} 
Before we delve into the proof, we want to point out to the reader that there is a small typo in the lemma statement in the main body. Instead of proving the statement for the point $\wh \w_t = \frac{1}{t} \sum_{\tau=1}^{t} \w_\tau$, in the following, we provide the proof for the average excess risk for the iterates $\crl{\w_\tau}_{\tau=1}^t$, i.e. $\En_{S}[\frac{1}{t} \sum_{\tau = 1}^t F({\w}^{}_{\tau})] - \inf_{\w \in \reals^d} F(\w) \ge \Omega(\beta_n)$. Furthermore, as we will see in the proof below, the same guarantee also holds for the last iterate $\w_t$. 

%\newcommand{\gdsuperscript}{\mathrm{GD}}
\newcommand{\gdsuperscript}{} 

\begin{proof} 
Recall that $n = O(\log(d))$. Consider the distribution $\cD = \cD(\frac{1}{4}, \frac{1}{2}, 0)$, given in \pref{def:violating_distribution_defn}, over the samples $z = (x, y, \alpha)$. Under this distribution note that the population loss $F(w) \ldef{} \En_{z \sim \cA} \brk*{f(\w; z)}$ is given by 
\begin{align*}
F(\w) &= \frac{3}{4} \left(\En_{x}\|\w \odot x\| \right) - \frac{1}{4}\left( \En_{x}\|\w \odot x\| \right)\\
&= \frac{1}{2} \En_{x}\|\w \odot x\|. 
\end{align*}
Hence, $F(\w) \le \frac{1}{2} \|\w\|$ and by Jensen's inequality, pushing expectation with respect to  $x$ inside, $F(\w) \ge \frac{1}{4} \|\w\|$. Let $\crl{\w_t}_{t \geq 1}$ denote the sequence of iterates generated by the GD algorithm, given in \pref{eq:GD}, with the starting point $\w_0$. From the gradient descent update we have
\begin{align*}
\w^{\gdsuperscript}_{t+1} &= \w^{\gdsuperscript}_t  -  \eta \cdot \frac{1}{n} \sum_{i=1}^n y_i \frac{ (\w^{\gdsuperscript}_t - \alpha ) \odot x_i}{\|(\w^{\gdsuperscript}_t - \alpha ) \odot x_i\|}\\ 
& = \w^{\gdsuperscript}_t  -  \eta \cdot \frac{1}{n} \sum_{i=1}^n y_i \frac{ \w^{\gdsuperscript}_t  \odot x_i}{\|\w^{\gdsuperscript}_t  \odot x_i\|}. 
\end{align*}
An application of \pref{lem:datatset_properties_basic_sco} implies that, for $n = O(\log(d))$, with probability at least $0.9$, there exists a coordinate $\hat{j}$ such that $x_i[\hat{j}] = 1$ whenever $y_i = -1$ and is 0 otherwise. Hence, on this coordinate, 
\begin{align*}
\abs[\big]{\w^{\gdsuperscript}_{t+1}[\hat{j}]} &= \abs[\Big]{\w^{\gdsuperscript}_t[\hat{j}]  +  \eta \cdot \frac{1}{n} \sum_{i: y_i = -1}  \frac{\w^{\gdsuperscript}_t[\hat{j}]}{\|\w^{\gdsuperscript}_t  \odot x_i\|}}\\
&\ge \abs[\big]{ \w^{\gdsuperscript}_t[\hat{j}] }\prn[\Big]{1  +  \eta  \cdot \frac{1}{n} \frac{\left| S^{-} \right| }{\|\w^{\gdsuperscript}_t \|}}, 
\end{align*}
where the set $S^- \ldef{} \crl*{z_i \in S:  y_i = -1}$. Now note that since $y_i$'s are $-1$ with probability $1/4$, we have that $\abs*{S^-} \geq \frac{n}{5}$ (by Hoeffding's inequality), specifically. This implies that % since the exapected value is $1/4$, with constant probability,
\begin{align*}
\abs[\big]{\w^{\gdsuperscript}_{t+1}[\hat{j}]} & \ge \abs[\big]{\w^{\gdsuperscript}_t[\hat{j}]} \prn[\Big]{1  +    \frac{\eta }{5 \|\w^{\gdsuperscript}_t \|}}.
\end{align*}
Hence we conclude that for any $t$,
\begin{align*} 
\abs[\big]{\w^{\gdsuperscript}_{t+1}[\hat{j}]}  & \ge \abs[\big]{ \w^{\gdsuperscript}_1[\hat{j}]} \prod_{\tau=1}^t \prn[\Big]{ 1  +    \frac{\eta }{ 5 \|\w^{\gdsuperscript}_\tau\|} } \\ & \ge \w^{\gdsuperscript}_1[\hat{j}] \prod_{\tau=1}^t 2^{ \frac{\eta}{5 \nrm{\w^{\gdsuperscript}_\tau} + \eta}} \\ % \frac{\frac{\eta }{ 4\|\w^{\gdsuperscript}_\tau \|}}{\left(1  +    \frac{\eta }{ 4\|\w^{\gdsuperscript}_\tau \|}\right)}}\\
& = \frac{1}{d^{1/2}} \prod_{\tau=1}^t 2^{\frac{\eta  }{\left(5 \|\w^{\gdsuperscript}_\tau \|  +  \eta \right)}}  =  2^{\sum_{\tau=1}^t \frac{\eta  }{\left(5 \|\w^{\gdsuperscript}_\tau \|  +  \eta \right)} - \frac{n}{2}}, 
\end{align*} where the inequality in the second last line holds from the fact that  $1+a \ge 2^{a/(1+a)}$ for $a \ge 0$. 
Noting that  $F(\w)$ is  lower bounded by $\frac{1}{4} \|\w\|$, the above implies that 
\begin{align*}
%\intertext{where in the above we used the fact that $1+x \ge 2^{x/(1+x)}$ for $x \ge 0$}
\abs[\big]{\w^{\gdsuperscript}_{t+1}[\hat{j}] } & \ge   2^{ \sum_{i=1}^t \frac{\eta  }{\left(20  F(\w^{\gdsuperscript}_\tau)  +  \eta \right)} - \frac{n}{2}}. 
\end{align*}
Note that $\abs{\w^{\gdsuperscript}_{t}[\hat{j}]}$ always increases. From this we can already conclude a few things. Note that $4 F(\w^{\gdsuperscript}_{t} ) \ge \left\|\w^{\gdsuperscript}_{t} \right\| \ge \abs{\w^{\gdsuperscript}_{t}[\hat{j}]}$. Hence, first we can conclude that for any $\Delta >0$, the number of iterations $\tau$ for which $ F(\w^{\gdsuperscript}_\tau) \le \Delta$ is at most $\frac{\left(20  \Delta  +  \eta \right)}{\eta}\left(\frac{n}{2} + \log_2(4 \Delta)\right)$. To see this note that, if at some iteration $m$ we have that $\left|\left\{\tau \le m : F(\w^{\gdsuperscript}_\tau) \le \Delta\right\}\right| = \frac{\left(20  \Delta  +  \eta \right)}{\eta}\left(\frac{n}{2} + \log_2(4 \Delta)\right)$, then note that for any $T \ge m$,
\begin{align*}
4 F(\w^{\gdsuperscript}_{T}) &\ge \abs[\big]{\w^{\gdsuperscript}_{k}[\hat{j}] } \\ & \ge 2^{ \sum_{i=1}^k \frac{\eta  }{\left(20  F(\w^{\gdsuperscript}_\tau)  +  \eta \right)} - \frac{n}{2}}\\
& \ge 2^{ \left|\left\{\tau \le m : F(\w^{\gdsuperscript}_\tau) \le \Delta\right\}\right| \left( \frac{\eta  }{\left(20  \Delta  +  \eta \right)}\right) - \frac{n}{2}}\\ 
& \ge 2^{ \left(\frac{n}{2} + \log_2(4 \Delta)\right) - \frac{n}{2}} = \Delta.
\end{align*}
Thus we can conclude that for any $T \ge m$, we have $F(\w^{\gdsuperscript}_{T}) > \Delta$. This implies that for any $\Delta$, the number of iterations $T$ such that $F(\w^{\gdsuperscript}_{T}) \le \Delta$ is at most $T \le \frac{\left(20  \Delta  +  \eta \right)}{\eta}\left(\frac{n}{2} + \log_2(4 \Delta)\right)$. Now from this we can conclude that for any $\Delta > 1/n$ (and $n > 4$ for instance), if  
\begin{align*}
T &> \frac{\left(20  \Delta  +  \eta \right)}{\eta}\left(\frac{n}{2} + \log_2(4 \Delta)\right)\\
&\ge \frac{n \left(20  \Delta  +  \eta \right)}{3 \eta}
\end{align*}
we can conclude that $F(\w^{\gdsuperscript}_{T}) \ge \Delta$. In the above, using $\Delta = \frac{3 \eta T}{20 n} - \frac{\eta}{20}$ we can conclude that, 
\begin{align*}
F(\w^{\gdsuperscript}_{T}) - \inf_{\w} F(\w) \ge \frac{1}{20}\left(\frac{3 \eta T}{n} - \eta \right)
\end{align*}

\end{proof}

\subsection{Proof of \pref{lem:gd_slow}}

\begin{proof} For this lemma, we pick the distribution $\cD$ where $x[1] = 1$ with probability $\delta$ for some $\delta > 1/\sqrt{n}$ that we will fix later and $x[1] = 0$ with probability $1- 
\delta$. We set $\alpha  = e_1$ deterministically and we also fix $y$ to be $+1$ deterministically.  We also pick $x[j]=0$ for all $j > 2$. 

Let $\crl{\w_t}_{t \geq 1}$ denote the sequence of iterates generated by the GD algorithm, given in \pref{eq:GD}, with the starting point $\w_0 \sim \cN(0, \frac{1}{d} \bbI_d)$.   Note that the optimal solution for $F(\w)$ is $\w = e_1$. However, for the initial point $\w_0$, with constant probability, $\w^{\gdsuperscript}_0[1] \leq 2/\sqrt{d} = 2^{-n/2}$. Further, on the first coordinate, each update step of GD algorithm is of the form 
\begin{align*}
\w^{\gdsuperscript}_{t+1}[1] &= \w^{\gdsuperscript}_{t}[1] - \eta \cdot \frac{1}{n} \sum_{i=1}^n \frac{(\w^{\gdsuperscript}_t[1] - 1)\odot x_i[1] }{\|(\w^{\gdsuperscript}_t - e_1) \odot x_i \|}\\
&= \w^{\gdsuperscript}_{t}[1] - \eta \cdot \frac{1}{n} \sum_{i=1}^n \frac{(\w^{\gdsuperscript}_t[1] - 1) \cdot x_i[1] }{|\w^{\gdsuperscript}_t[1] - 1|}\\
&= \w^{\gdsuperscript}_{t}[1] - \eta \cdot \frac{1}{n} \sum_{i: x_i[1] = 1} \frac{(\w^{\gdsuperscript}_t[1] -1)}{|\w^{\gdsuperscript}_t[1] -1|}\\
&= \w^{\gdsuperscript}_{t}[1] - \eta \cdot \mathrm{sign}(\w^{\gdsuperscript}_{t}[1] - 1) \cdot \frac{1}{n} \left| S_1\right|,  \numberthis \label{eq:GD_update_rule}
\end{align*}
where the set $S_1 \ldef{} \left\{z_i \in S: x_i[1] = 1\right\}$. Note that with high probability $\frac{1}{n}  \left| S_1 \right| \le \delta + \frac{1}{\sqrt{n}}$ and so if $\delta > 1/\sqrt{n}$ then we have that with constant probability, $\abs{S_1} \le 2 \delta n$. Further, since $\w^{\gdsuperscript}_1[1] \le \frac{2}{\sqrt{d}}$ with constant probability, the above update rule in \pref{eq:GD_update_rule} implies that 
\begin{align} 
|\w^{\gdsuperscript}_{t+1}[1]| & \le |\w^{\gdsuperscript}_{t}[1]| + \eta \cdot \frac{1}{n} \abs{S_1} \notag\\
& \le   |\w^{\gdsuperscript}_{t}[1]| + 2 \eta \delta\notag\\
& \le   \frac{2}{\sqrt{d}} + 2 \eta \delta t. \label{eq:one}
\end{align}
Next, note that $F(\w) = \delta |\w[1] - 1|$ and so if we want $F(\w) - \inf_{\w} F(\w) \le \delta/2$ then, it should be that $ |\w[1] - 1| \le\frac{1}{2}$, and so 
$|\w^{\gdsuperscript}_{t+1}[1]| > 1/2$. Using this with \pref{eq:one} we need that 
$$
 \frac{2}{\sqrt{d}} + 2 \eta \delta t > 1/2
$$
Thus, from the contrapositive, we have that if $t \eta < \left(1/2 - \frac{1}{2^{n/2}}\right)/{2 \delta}$, then $$F(\w^{\gdsuperscript}_t) - \inf_{\w} F(\w) > \delta/2.$$ Further note that if instead of $\w^{\gdsuperscript}_t$ we take the average iterate $\widehat{\w}^{\gdsuperscript}_t$, the norm only reduces since in each iteration we are increasing the magnitude and thus the last iterate has the largest magnitude. This implies that the average iterate $\wh \w$ also satisfies 
$$F(\wh \w^{\gdsuperscript}_t) - \inf_{\w} F(\w) > \delta/2.$$
Using the $\eta$ and number of iterations $t$ from the lemma, we can conclude the statement. 
\end{proof}






==> files/sec_GDvsSGD_old.tex <==
%!TEX root=../paper.tex
In the previous section, we provided a construction on which no regularized ERM works as well as SGD. When gradient descent algorithm (specified in  \pref{eq:GD}) is used for training, one would expect that GD, and in general large batch SGD, will eventually converge to an ERM and so after enough iterations would also fail to find a good solution. In this section, we provide precise expressions for how fast GD on training loss begins to diverge from the desired solution (population minimizer).  

\begin{lemma}
\label{lem:lem1_main_gdvssgd}
For the function $f_{(\ref{eq:empfn_basic_cons_sco})}$ specified in Equation (\ref{eq:empfn_basic_cons_sco}), there exists a distribution $\cD \in \convexclass$ s.t., for any step size $\eta$,  if number of iterations $t$ is larger than $\frac{n}{2} + \Omega(\frac{2 n \beta_n}{\eta})$ then 
$$
\En_{S}[F(\widehat{\w}^{\mathrm{GD}}_{t})] - \inf_{\w \in \reals^d} F(\w) \ge \Omega(\beta_n) 
$$ 
\end{lemma}

The above lemma basically tells us that for any step size, the excess risk of gradient descent algorithm eventually is lower bounded by a constant. For instance, if we set $\beta_n$ to be a constant, then excess risk of GD is $\Omega(1)$, once number of iterations exceeds $O(n / \eta)$. The same lemma also implies the following corollary that tells us that as soon as the number of iterations exceed order $n$, excess risk of the point returned by GD is worse than that of SGD. 

To give a sketch of why the above lemma holds, note that as earlier, when $d > 2^n$ with constant probability there is a coordinate $\wh j$ such that $x_t[\wh j] = 1$ whenever $y_t = -1$ and is 0 otherwise. Hence for this coordinate, we notice that GD update is of form $$\w^{\mathrm{GD}}_{t+1}[\wh j] \ge \w^{\mathrm{GD}}_{t}[\wh j] (1 + \frac{\eta}{4 \|\w^{\mathrm{GD}}_t\|_2}).$$ Completing the recursion, we get that  $$\w^{\mathrm{GD}}_{t+1}[\wh j] \ge \w^{\mathrm{GD}}_1[\wh j] \prod_{i=1}^t (1 + \frac{\eta}{4\|\w^{\mathrm{GD}}_i\|_2}).$$ Noting that if $\|\w^{\mathrm{GD}}_i\|_2$ on average is of order $\beta_n$ and since $\w^{\mathrm{GD}}_1[\wh j] $ is of order $1/\sqrt{d}= 2^{-n/2}$ we can obtain a bound on how large $t$ can be before $\w^{\mathrm{GD}}_t[\wh j]$ becomes as large as a constant.\footnote{Throughout the paper, we use the standard non-asymptotic big-$O$, big-$\Omega$, little-$o$ and little-$\omega$ notation. }
 
\begin{corollary}
For the function $f_{(\ref{eq:empfn_basic_cons_sco})}$ specified in Equation (\ref{eq:empfn_basic_cons_sco}), and for any step size $\eta =\Omega(1/\sqrt{n})$ and any $t > \Omega(n)$, there exists a distribution $\cD \in \convexclass$ s.t.,
$$ 
\En_{S}[F(\widehat{\w}^{\mathrm{GD}}_{t})] - \inf_{\w \in \reals^d} F(\w) \ge \omega\prn[\Big]{\frac{1}{\sqrt{n}}}. %\Omega\left(\frac{1}{\sqrt{n}}\right)
$$ 
\end{corollary} 

The above corollary says that when step size is $1/\sqrt{n}$ or larger, then as soon as number of iterations is larger than order $n$, GD has excess risk lower bounded by $\omega(1/\sqrt{n})$. We complement this corollary with the following lemma that says that if the step size is smaller than order $1/\sqrt{n}$, then if GD is run for less than order $n$ number of iterations, its excess risk is again lower bounded by $\omega(1/\sqrt{n})$.

\begin{lemma}\label{lem:gd_slow}
For the function $f_{(\ref{eq:empfn_basic_cons_sco})}$ specified in Equation (\ref{eq:empfn_basic_cons_sco}), and for any step size $\eta = o(1/\sqrt{n})$ and any $t = O(n)$, there exists a distribution $\cD \in \convexclass$ such that,
$$
\En_{S}[F(\widehat{\w}^{\mathrm{GD}}_{t})] - \inf_{\w \in \reals^d} F(\w) \ge \omega\prn[\Big]{\frac{1}{\sqrt{n}}}. 
$$
\end{lemma} 

The above lemma tells us that if step size is too small (smaller than $1/\sqrt{n}$) then GD will also take too long (more than $n$ iterations) to converge. 

\begin{remark}
Note that as mentioned in \pref{prop:nn}, the function $f_{(\ref{eq:empfn_basic_cons_sco})}$ can be represented as a simple restricted neural network. Hence this example also shows us that GD does not work for deep learning models as well.
\end{remark}

The results in this section not only suggests that GD is worse than SGD, but also that GD will in fact not even learn if run for too long. Specifically, It diverges to a constant excess risk point in $n^{3/2}$ iterations (set $\eta = 1/\sqrt{n}$ in \pref{lem:lem1_main_gdvssgd}), and has strictly worse than $1/\sqrt{n}$ excess risk in $\Omega(n)$ rounds. In the next section we provide insight into when multi-pass SGD can provide better guarantees which combined with this result tells us that while many rounds of GD might not be good, multi-pass SGD as given in the procedure in the next section can help improve performance. 

\begin{remark} 
Using the function $f_{(\ref{eq:empfn_basic_cons})}$, given in \pref{sec:SGDimp}, we can also provide an example in the distribution free learnable setting where SGD outperforms GD. %is outperformed by SGD.
\end{remark}

\ascomment{GD with validation} 







==> files/sec_beyondSCO.tex <==
\subsection{Beyond Stochastic Convex Optimization}
\begin{definition}[$\epsilon$-linearizable functions] 
	
\end{definition} 

\begin{theorem}[SGD works for $\epsilon$-linearizable networks] 
	
\end{theorem} 

\begin{theorem}[SGD works but with projection]  
	
\end{theorem}


==> files/sec_gd_temp.tex <==

%!TEX root=../paper.tex
In the previous section, we showed that no regularized ERM works for the construction given there. When gradient descent algorithm (specified in Eq. \ref{eq:GD} is used, one would expect that eventually GD (and in general large batch SGD) converges to ERM and so after enough iteration probably also fails. In this section, we provide precise expression for how fast GD on training loss begins to diverge from the desired solution (population minimizer). 


\begin{lemma}
For the function $f_{(\ref{eq:empfn_basic_cons_sco})}$ specified in Equation (\ref{eq:empfn_basic_cons_sco}), there exists a distribution $\cD \in \convexclass$ s.t., for any step size $\eta$,  if number of iterations $t$ is larger than $\frac{n}{2} + \Omega(\frac{2 n \beta_n}{\eta})$ then 
$$
\En_{S}[F(\widehat{\w}^{\mathrm{GD}}_{t})] - \inf_{\w \in \reals^d} F(\w) \ge \Omega(\beta_n)
$$
\end{lemma}

The above lemma basically tells us that for any step size, the excess risk of gradient descent algorithm eventually is lower bounded by a constant. For instance, if we set $\beta_n $ to be a constant, then excess risk of GD is lower bounded by a constant once number of iterations exceeds order $\frac{n}{\eta}$. The same lemma also implies the following corollary that tells us that as soon as number of iterations exceeds order $n$, excess risk of gradient descent is worse than that of SGD.

To give a sketch of why the above lemma holds, note that as earlier, when $d > 2^n$ with constant probability there is a coordinate $\hat{j}$ such that $x_t[\hat{j}] = 1$ whenever $y_t = -1$ and is 0 otherwise. Hence for this coordinate one notices that GD update is of form that $\w^{\mathrm{GD}}_{t+1}[\hat{j}] \ge \w^{\mathrm{GD}}_{t}[\hat{j}] (1 + \frac{\eta}{4 \|\w^{\mathrm{GD}}_t\|_2})$. Thus completing the recursion we get that  $\w^{\mathrm{GD}}_{t+1}[\hat{j}] \ge \w^{\mathrm{GD}}_1[\hat{j}] \prod_{i=1}^t (1 + \frac{\eta}{4\|\w^{\mathrm{GD}}_i\|_2})$. Noting that if $\|\w^{\mathrm{GD}}_i\|_2$ on average is of order $\beta_n$ and since $\w^{\mathrm{GD}}_1[\hat{j}] $ is of order $1/\sqrt{d}= 2^{-n/2}$ we can obtain a bound on how large $t$ can be before the bad coordinate of $\w^{\mathrm{GD}}_t$ becomes as large as a constant.
 
\begin{corollary}
and for any step size $\eta =\Omega(1/\sqrt{n})$ and any $t > \Omega(n)$, there exists a distribution $\cD \in \convexclass$ s.t.,
$$
\En_{S}[F(\widehat{\w}^{\mathrm{GD}}_{t})] - \inf_{\w \in \reals^d} F(\w) \ge \omega\left(\frac{1}{\sqrt{n}}\right)
$$
\end{corollary}

The above corollary says that when step size is $1/\sqrt{n}$ or larger, then as soon as number of iterations is larger than order $n$, GD has excess risk lower bounded by $\omega(1/\sqrt{n})$. We complement this corollary with the following lemma that says that if step size if smaller than order $1/\sqrt{n}$, then if GD is run for less than order $n$ number of iterations, its excess risk is again lower bounded by $\omega(1/\sqrt{n})$.

\begin{lemma}
For any step size $\eta = o(1/\sqrt{n})$ and any $t = O(n)$, there exists a distribution $\cD \in \convexclass$ such that,
$$
\En_{S}[F(\widehat{\w}^{\mathrm{GD}}_{t})] - \inf_{\w \in \reals^d} F(\w) \ge \omega\left( \frac{1}{\sqrt{n}}\right)
$$
\end{lemma}

The above lemma tells us that if step size is too small (smaller than $1/\sqrt{n}$) then GD will also take too long (more than $n$ iterations) to converge. 


The results in this section tells us not only that GD is worse than SGD but also that GD will in fact not even learn if run for too long. It completely diverges to constant excess risk in $n^{3/2}$ iterations and has worse than $1/\sqrt{n}$ excess risk in $\Omega(n)$ rounds. In the next section we provide insight into when multi-epoch SGD can provide better guarantees which combined with this result tells us that while many rounds of GD might not be good, multi-epochs of SGD as given in the procedure in the next section can help improve performance.


==> files/sec_sco.tex <==
%!TEX root=../neurips_2021.tex
A stochastic optimization problem has the form:
\begin{align}
\mathrm{Minimize}~~ F(w)
 \end{align}
where the $F(w) = \En_{z \sim D} \brk*{f(w; z)}$  based only on samples $z_1,\ldots,z_n$ drawn i.i.d. from the distribution $D$. Perhaps the most well studied instance of stochastic optimization problem is the Stochastic Convex Optimization (SCO) where the objective $F:\reals^d \mapsto \reals$ is convex. A standard assumption made for SCO problems, which we also make in this work is that:
$$
\exists \w^\star \in \argmin_{\w} F(w) \textrm{ s.t. }\|\w^\star\|_2 \le 1
$$
and that 
$$
\max\{ \En_{z \sim D} \|\nabla f(w,z) - \nabla F(w)\|^2 ~,~ \En_{z \sim D} \|\nabla f(w,z)\|^2\} \le \sigma^2 
$$
We note that while the objective $F$ is assumed to be convex, we don't necessarily assume that for each sample $z$, $f(\cdot,z)$ is a convex function. We only assume that $f(\cdot,z)$ has sub or super gradients at every point which we denote by $\nabla f(\w,z)$. Indeed, stochastic first order algorithms like stochastic gradient descent algorithms don't need such convexity of every $f(\cdot,z)$ to guarantee convergence but only require that objective $F$ is convex. 

% \clearpage   
%We consider the general learning setting \citep{vapnik2013nature} where we would like to minimize the population risk:
%$$
%F(\w) = \En_{z \sim \cD}\left[ f(\w; z)\right], 
%$$
%where $f : \reals^d \times \cZ \mapsto \reals$ is the instantaneous loss function, $\w \in \reals^d$ parameterizes the model used for learning and the distribution $\cD$ on $\cZ$ is a distribution over instance space that is unknown to the learner. The learner only has access to samples $S = \{z_1,\ldots,z_n\}$ drawn iid from $\cD$. The goal of the learner is to return a model $\widehat{\w} \in \reals^d$, based on a sample of size $n$, with as small a population risk as possible. 


Specifically, we say that an algorithm is $\epsilon$ sub-optimal if
$$\En_{S}[F(\widehat{\w})] - \inf_{\w \in \W} F(\w) \le \epsilon,$$
where the expectation above is over samples and $\W$ is a set of feasible solutions. Several algorithms have been proposed and studied for the problem of Stochastic convex optimization. Perhaps the most well known of these are, gradient descent, stochastic gradient descent and regularized ERM. We describe each of these methods below.

%It is worth noting that most statistical learning problems can be encoded in the above setting. As a specific example, $\w \in \reals^d$ could encode the weights of a neural network and $\cZ = \cX \times \cY$ could encode the input instances in $\cX$ and labels or output in $\cY$. The function $f(\w;z)$ then simply corresponds to the loss on example $z$ for the neural network with weights specified by $\w$.

\paragraph{(Regularized) Empirical Risk Minimization.} Perhaps the simplest algorithm one could consider is the Empirical Risk Minimization (ERM) algorithm where one simply returns a minimizer of empirical risk $F_S(\w) \ldef{} \frac{1}{n} \sum_{t=1}^n f(\w;z_t)$. That is,
$\w_{\mathrm{ERM}} \in \argmin_{\w \in \W} F_S(\w)$.
There are several problems for which ERM algorithm in general might successfully finds a solution with low population level sub-optimality. Typically in these problems one has uniform convergence, in the sense that for every $\w \in \W$, $|F_S(\w)- F(\w)|$ converges to $0$ as $n$ increases (in expectation or high probability). However, it is well known that ERM might fail in general \citep{shalev2009stochastic, feldman2016generalization}. In \citet{shalev2009stochastic} an instance of a problem where ERM does not work, yet either SGD or Regularized ERM (RERM) have provably diminishing excess risk, is provided. Thus showing that ERM is not a universal algorithm and that uniform convergence is not necessary for learnability. While in \citet{shalev2009stochastic} the dimensionality of the problem is very large, in \citet{feldman2016generalization} the result is shown to hold even when dimensionality of the problem is of the same order as number of training samples. While these works show that ERM fails, they do not however exclude RERM as a universal algorithm. RERM is given by 
$$
\w_{\mathrm{RERM}} = \argmin_{\w \in \W} F_S(\w)  + R(\w)
$$
where $R: \reals^d \mapsto \reals$ is a regularization function. 

\paragraph{Gradient Descent (GD).} Gtradient descent algorithm on training loss is one that performs the following update on every iteration:
\begin{align}\label{eq:GD}
\w^{\mathrm{GD}}_{t+1} \leftarrow \w^{\mathrm{GD}}_{t} - \eta \nabla F_S(\w^{\mathrm{GD}}_{t}),
\end{align}
where $\eta$ denotes the step size. We can consider two variants: (a) the widely used last iterate variant where on iteration $t$ one simply returns $\w^{\mathrm{GD}}_{t}$, and (b) the averaging variant commonly used for convex problems that on round $t$ returns the average iterate $\widehat{\w}^{\mathrm{GD}}_{t} \ldef{} \frac{1}{t} \sum_{i=1}^t\w^{\mathrm{GD}}_{i}$. 

\paragraph{Stochastic Gradient Descent (SGD).}
Single pass SGD algorithm runs for $n$ steps and for each step takes a single data point and performs gradient update w.r.t. that sample. That, is on round $t$,
\begin{align}\label{eq:SGD}
\w^{\mathrm{SGD}}_{t+1} \leftarrow \w^{\mathrm{SGD}}_{t} - \eta \nabla f(\w^{\mathrm{SGD}}_t;z_t) 
\end{align} 
Finally, we return $\widehat{\w}^{\mathrm{SGD}}_t = \frac{1}{t} \sum_{i=1}^t \w^{\mathrm{SGD}}_{i}$.

%\paragraph{Stochastic Convex Optimization (SCO).} When population risk $F$ is convex in $\w$, the problem is often referred to as stochastic convex optimization. When $F$ is convex and $L$-Lipchitz, then it is well known that single pass SGD enjoys a sub-optimality rate of $O(\frac{L}{\sqrt{n}})$. For a given problem, we shall use the notation $\convexclass$ to denote the set of distributions over instances for which the population loss is convex, and thus the problem is an instance of an SCO problem. Specifically, 
%\begin{align}\label{eq:convdis} 
%\convexclass \ldef{} \crl*{\cD \mid F(\w) = \En_{z \sim \cD} \brk*{f(\w, z)} \text{ is convex in $\w$}}. 
%\end{align} 
%
%\ascomment{Add the $w^*$ part here!} 

 \paragraph{Initial Weights.}
Throughout this paper we assume that the initial weights $w_0$ are chosen by first drawing $\w'_0 \sim \mathcal{N}(0, \bbI_d/d)$ and then setting $w_0 = w'_0 / \nrm*{w'_0}$ to ensure bounded initial weights.  %the standard initialization in deep learning.  

\paragraph{Notation.}
 For a vector $\w \in \bbR^d$, $\nrm{\w}$ denotes the Euclidean norm and $\nrm{\w}_\infty$ denotes the $\ls_\infty$ norm. The notation $\w[j]$ denotes the $j$-th coordinate of the vector $\w$.  We adopt the non-asymptotic big-$O$ notation, where $f = O(g)$ for $f, g: \cW \mapsto \bbR^+$ if $f(w) \leq Cg(w)$ for some constant $C > 0$. Similarly, the non-asymptotic  big-$\Omega$ notation, little-$o$ notation and little-$\omega$ notation follow the standard definitions.  

% \paragraph{Notation.} For a vector $\w \in \bbR^d$, $\nrm{\w}$ denotes the Euclidean norm and $\nrm{\w}_\infty$ denotes the $\ls_\infty$ norm. The notation $\w[j]$ denotes the $j$-th coordinate of the vector $\w$. We adopt the non-asymptotic big-$O$ notation, where $f = O(g)$ for $f, g: \cW \mapsto \bbR^+$ if $f(w) \leq Cg(w)$ for some constant $C > 0$. Similarly, the non-asymptotic  big-$\Omega$ notation, little-$o$ notation and little-$\omega$ notation has the standard definitions, as in the optimization literature.
 
  % is defined as the standard used in the literature. %The non-asymptotic big-$\Omega$ notation is defined such that $f = \Omega(g)$ iff $g = O(f)$. Similarly, we define the non-asymptotic little-$o$ notation,  such that $f = o(g)$ if for any constant $c > 0$, there exists some $x_0$ such that $f(x) \leq c g(x)$ for all $x \geq x_0$. Similarly, we define the little-$\omega$ notation such that $f = \omega(g)$ iff $g = o(f)$. 
  

==> files/sec_setup.tex <==
%!TEX root=../paper.tex

\section{Preliminaries (OLD)} 
We consider the general learning setting \citep{vapnik2013nature} where we would like to minimize the population risk:
$$
F(\w) = \En_{z \sim \cD}\left[ f(\w; z)\right], 
$$ 
where $f : \reals^d \times \cZ \mapsto \reals$ is the instantaneous loss function, $\w \in \reals^d$ parameterizes the model used for learning and the distribution $\cD$ on $\cZ$ is a distribution over instance space that is unknown to the learner. The learner only has access to samples $S = \{z_1,\ldots,z_n\}$ drawn iid from $\cD$. The goal of the learner is to return a model $\widehat{\w} \in \reals^d$, based on a sample of size $n$, with as small a population risk as possible. Specifically, we say that an algorithm is $\epsilon$ sub-optimal if
$$\En_{S}[F(\widehat{\w})] - \inf_{\w \in \W} F(\w) \le \epsilon,$$
where the expectation above is over samples and $\W$ is a set of feasible solutions. It is worth noting that most statistical learning problems can be encoded in the above setting. As a specific example, $\w \in \reals^d$ could encode the weights of a neural network and $\cZ = \cX \times \cY$ could encode the input instances in $\cX$ and labels or output in $\cY$. The function $f(\w;z)$ then simply corresponds to the loss on example $z$ for the neural network with weights specified by $\w$.

\paragraph{(Regularized) Empirical Risk Minimization.} Perhaps the simplest algorithm one could consider is the Empirical Risk Minimization (ERM) algorithm where one simply returns a minimizer of empirical risk $F_S(\w) \ldef{} \frac{1}{n} \sum_{t=1}^n f(\w;z_t)$. That is,
$\w_{\mathrm{ERM}} \in \argmin_{\w \in \W} F_S(\w)$.
There are several problems for which ERM algorithm in general might successfully finds a solution with low population level sub-optimality. Typically in these problems one has uniform convergence, in the sense that for every $\w \in \W$, $|F_S(\w)- F(\w)|$ converges to $0$ as $n$ increases (in expectation or high probability). However, it is well known that ERM might fail in general \citep{shalev2009stochastic, feldman2016generalization}. In \citet{shalev2009stochastic} an instance of a problem where ERM does not work, yet either SGD or Regularized ERM (RERM) have provably diminishing excess risk, is provided. Thus showing that ERM is not a universal algorithm and that uniform convergence is not necessary for learnability. While in \citet{shalev2009stochastic} the dimensionality of the problem is very large, in \citet{feldman2016generalization} the result is shown to hold even when dimensionality of the problem is of the same order as number of training samples. While these works show that ERM fails, they do not however exclude RERM as a universal algorithm. RERM is given by 
$$
\w_{\mathrm{RERM}} = \argmin_{\w \in \W} F_S(\w)  + R(\w)
$$
where $R: \reals^d \mapsto \reals$ is a regularization function. 

\paragraph{Gradient Descent (GD).} Gtradient descent algorithm on training loss is one that performs the following update on every iteration:
\begin{align}\label{eq:GD}
\w^{\mathrm{GD}}_{t+1} \leftarrow \w^{\mathrm{GD}}_{t} - \eta \nabla F_S(\w^{\mathrm{GD}}_{t}),
\end{align}
where $\eta$ denotes the step size. We can consider two variants: (a) the widely used last iterate variant where on iteration $t$ one simply returns $\w^{\mathrm{GD}}_{t}$, and (b) the averaging variant commonly used for convex problems that on round $t$ returns the average iterate $\widehat{\w}^{\mathrm{GD}}_{t} \ldef{} \frac{1}{t} \sum_{i=1}^t\w^{\mathrm{GD}}_{i}$. 

\paragraph{Stochastic Gradient Descent (SGD).}
Single pass SGD algorithm runs for $n$ steps and for each step takes a single data point and performs gradient update w.r.t. that sample. That, is on round $t$,
\begin{align}\label{eq:SGD}
\w^{\mathrm{SGD}}_{t+1} \leftarrow \w^{\mathrm{SGD}}_{t} - \eta \nabla f(\w^{\mathrm{SGD}}_t;z_t) 
\end{align} 
Finally, we return $\widehat{\w}^{\mathrm{SGD}}_t = \frac{1}{t} \sum_{i=1}^t \w^{\mathrm{SGD}}_{i}$.

\paragraph{Stochastic Convex Optimization (SCO).} When population risk $F$ is convex in $\w$, the problem is often referred to as stochastic convex optimization. When $F$ is convex and $L$-Lipchitz, then it is well known that single pass SGD enjoys a sub-optimality rate of $O(\frac{L}{\sqrt{n}})$. For a given problem, we shall use the notation $\convexclass$ to denote the set of distributions over instances for which the population loss is convex, and thus the problem is an instance of an SCO problem. Specifically, 
\begin{align}\label{eq:convdis} 
\convexclass \ldef{} \crl*{\cD \mid F(\w) = \En_{z \sim \cD} \brk*{f(\w, z)} \text{ is convex in $\w$}}. 
\end{align} 

\ascomment{Add the $w^*$ part here!} 

 \paragraph{Initial Weights.}
Throughout this paper we assume that the initial weights $w_0$ are chosen by first drawing $\w'_0 \sim \mathcal{N}(0, \bbI_d/d)$ and then setting $w_0 = w'_0 / \nrm*{w'_0}$ to ensure bounded initial weights.  %the standard initialization in deep learning.  

\paragraph{Notation.}
 For a vector $\w \in \bbR^d$, $\nrm{\w}$ denotes the Euclidean norm and $\nrm{\w}_\infty$ denotes the $\ls_\infty$ norm. The notation $\w[j]$ denotes the $j$-th coordinate of the vector $\w$.  We adopt the non-asymptotic big-$O$ notation, where $f = O(g)$ for $f, g: \cW \mapsto \bbR^+$ if $f(w) \leq Cg(w)$ for some constant $C > 0$. Similarly, the non-asymptotic  big-$\Omega$ notation, little-$o$ notation and little-$\omega$ notation follow the standard definitions.  

% \paragraph{Notation.} For a vector $\w \in \bbR^d$, $\nrm{\w}$ denotes the Euclidean norm and $\nrm{\w}_\infty$ denotes the $\ls_\infty$ norm. The notation $\w[j]$ denotes the $j$-th coordinate of the vector $\w$. We adopt the non-asymptotic big-$O$ notation, where $f = O(g)$ for $f, g: \cW \mapsto \bbR^+$ if $f(w) \leq Cg(w)$ for some constant $C > 0$. Similarly, the non-asymptotic  big-$\Omega$ notation, little-$o$ notation and little-$\omega$ notation has the standard definitions, as in the optimization literature.
 
  % is defined as the standard used in the literature. %The non-asymptotic big-$\Omega$ notation is defined such that $f = \Omega(g)$ iff $g = O(f)$. Similarly, we define the non-asymptotic little-$o$ notation,  such that $f = o(g)$ if for any constant $c > 0$, there exists some $x_0$ such that $f(x) \leq c g(x)$ for all $x \geq x_0$. Similarly, we define the little-$\omega$ notation such that $f = \omega(g)$ iff $g = o(f)$. 
  

==> files/sgd_and_implicit_regularization.tex <==
In \citet{shalev2009stochastic} (see also \cite{feldman2016generalization}), SCO problems where not just the population loss $F$ but where also for each $z \in \cZ$, the instantaneous loss $f(\cdot,z)$ is convex is considered. In this setting, the authors show that the appropriate $\ell_2$ norm square regularized RERM always obtains the optimal rate of $1/\sqrt{n}$. However, for SGD to obtain a $1/\sqrt{n}$ guarantee, one only needs convexity at the population level.   In this section, based on construction of SCO problems that are convex only at population level and not at the empirical level, we show a strict separation between SGD and RERM. Specifically, while SGD is always successful for any SCO problem we consider here, we show that for any regularizer $R$, there is an instance of an SCO problem for which RERM w.r.t. this regularizer has suboptimality lower bounded by a constant. 

==> files/temp_files/app_RERM_basic_proof_old.tex <==
\subsection{Proof of \pref{thm:lowersco}}  \label{app:thm_lowersco_proof} 
We now have all the tools required to prove \pref{thm:lowersco}, which states that no regularization function $R(\w)$ succeeds to find an $\epsilon$-suboptimal solution, with probability at least $0.9$, for all distributions in the class $\convexclass$. 

% \begin{definition} \label{def:violating_distribution_defn_a}
% For parameters $\delta \in [0, \frac{1}{2}]$, $p \in [0, 1]$, and $v \in \bbR^d$, define the distribution $\cD(\delta, p, v)$ over $z = (x, y, \alpha)$ as follows:
% \begin{align*} x \sim \text{Bernoulli}\prn*{p}^d, \qquad y \sim \text{Bernoulli}(\tfrac{1}{2} + \delta) \quad \text{and} \quad \alpha = v.
% \end{align*}
% The components $x$, $y$ and $\alpha$ are sampled independently.
% \end{definition} 

% Let $\cB(p)$ denotes the Bernoulli distribution with $\Pr(1) = p$.

% The following lemma shows that any such distribution $\cD(\delta, p, a)$ belongs to the class $\convexclass'$. 
\begin{proof}[{\bf Proof of \pref{thm:lowersco}} ]  
% \skcomment{Change $w \to \w$ in the proof below.}
Suppose there exists a regularization $R: \bbR^d \to \bbR$ and an $\epsilon < \frac{1}{20}$ such that for any distribution $\cD \in \convexclass$, the regularized ERM algorithm with regularization $R(\w)$ finds, with probability at least $0.9$ over the choice of the training set $S$, an $\epsilon$-suboptimal solution with respect to the test loss $F(\w) = \En_{z \in \cD} \brk*{f(\w, z)}$. We will show that $\epsilon$ must be greater than $1/1200$ which proves the theorem. %implies the statement of the lemma.

In order to prove so, we will consider two distributions $\cD_1$ and $\cD_2$, both of which are in $\convexclass$. We will work in the setting where $n \leq O(\log(d))$ with $d$ being the problem dimension. We will also assume that $n \geq 500$. In the proof, we will show that the assumed performance guarantee of RERM for $\cD_1$, and $\cD_2$ respectively, imply a certain lower bound on the value of $\epsilon$ which depends on the structure of the regularization function $R$. Combining the two lower bounds that we get from the analysis for $\cD_1$ and $\cD_2$ given us a lower bound on $\epsilon$ which is free from the structure of the regularization function $R$, hence proving the desired claim. 

\paragraph{Setup:} We first note that by \pref{lem:pop-loss-convexity}, for any distribution $\cD(\delta, \tfrac{1}{2}, a)$, defined in \pref{def:violating_distribution_defn}, any $\epsilon$-suboptimal minimizer $\w$ for the test loss $F$ must satisfy 
\begin{align*}
\|\w - a\| \leq \frac{\epsilon}{\delta}. \numberthis \label{eq:rerm_doesnt_work10} 
\end{align*} 
% To see this, note that 
% \begin{align*}
% F(\w') = 2\delta \En_{x} \brk*{\nrm*{(\w' - v) \odot x}} \geq 2\delta \nrm*{(\w' - v) \odot \En_{x}[x]} = \delta\nrm*{w' - v},  
% \end{align*}
% where the second inequality follows from Jensen's inequality, and the last equality from the fact that $x \sim \text{Bernoulli}(\frac{1}{2})^d$. Using the fact that $F(\w') - \min_w F(\w) \leq \epsilon$ and that $\min_{w} F(\w) = 0$, we get the above bound on $\|w' - v\|$. % \leq \frac{\epsilon}{\delta}$.

Further, let us define some additional notation. For convenience, set $e_0 = 0$, and define the points $\w^*_j$ for $j \in \{0, 1, \ldots, d\}$ as follows: %Motivated by this observation, define 
\begin{align*} 
\w^*_{j}  \in \argmin_{\w:\ {\nrm*{\w - e_j} \leq 10\epsilon}} R(\w).  \numberthis \label{eq:w_jstar_defn} 
\end{align*} 
Additionally, let the index $j^* \in [d]$ be defined such that $j^* \in \argmax_{j \in [d]} ~ R(\w^*_j)$. 

% Note that the distributions $\cD_j$ for $j \in \{0, 1, \ldots, d\}$ have the same marginal distribution on $(x, y)$ and only differ in the deterministic choice of $\alpha$. So sampling a dataset $S$ from any given $\cD_j$ is equivalent to sampling $(x, y)$ from the shared marginal distribution, and then choosing $\alpha = e_j$ for all the sampled $(x, y)$ pairs.

\paragraph{Distribution-1:} Suppose we sample a datatset  $S$ of size $n$ from the distribution $\cD_1 := \cD(\frac{1}{4}, \frac{1}{2}, 0)$. The assumed performance guarantee of RERM implies that, with probability at least $0.9$, RERM  algorithm on the dataset $S$ returns an $\epsilon$-suboptimal minimizer of the population loss $F_1(\w) = \En_{z \sim \cD_1} \brk*{f(\w, z)}$ under $\cD_1$. Let the sets $S^+$ and $S^-$ be defined such that 
\begin{align*}
   S^+ &\ldef{} \crl*{z_i  \in S \mid{} y_i = +1} \\ 
   S^- &\ldef{} \crl*{z_i \in S \mid{} y_i = -1}.  \numberthis \label{eq:set_plus_minus_definition} 
\end{align*}
%as defined in \pref{eq:set_plus_minus_definition}. 
Using Hoeffding's inequality, with probability at least $0.9$, $|S^{-}| \geq \frac{n}{5}$. Next, using \pref{lem:datatset_properties_basic_sco}, we have that, with probability at least $0.9$, there exists a special coordinate $\wh j \in [d]$ such that $x[\wh j]= 0$ for all $z \in S^{+}$ and $x[\wh j]= 1$ for all $z \in S^{-}$. This implies that, with probability at least $0.7$, all three events happen (i.e. RERM returns an $\epsilon$-suboptimal solution, $|S^{-}| \geq \frac{n}{5}$, and there is a special coordinate $\wh j$ for $S$ as described above). Henceforth we condition on the occurrence of these events. %sIn the following, we condition on the fact that his event holds. \ascomment{Fix statement} 

Consider the point $\w^*_{\wh j}$ defined in \pref{eq:w_jstar_defn} for the special coordinate $\wh j$. Since $\|\w^*_{\wh j} - e_{\wh j}\| \leq 10\epsilon$, we have $$\|\w^*_{\wh j}\| \geq 1 - 10\epsilon > 10\epsilon.$$ 
However, note that any $\epsilon$-suboptimal point $w$ with respect to $F_1(\w)$ must satisfy \pref{eq:rerm_doesnt_work10}, which in this case corresponds to the condition that  $\|w\| \leq \epsilon / \delta = 10\epsilon$.  This implies that $\w^*_{\wh j}$ cannot be an $\epsilon$-suboptimal minimizer of $F_1$, and thus $\w^*_{\wh j}$ can not be a minimizer of the regularized empirical risk (as all RERM solutions are $\epsilon$-suboptimal w.r.t. the population loss $F_1$). Using $\wh F_1$ to denote the empirical loss on $S$, we get that 
\begin{align*} 
\wh F_1(\w^*_{\wh j}) + R(\w^*_{\wh j}) &> \min_{\w:\ \|\w\| \leq 10\epsilon} \prn*{\wh F_1(\w) + R(\w)} \\ &\geq \min_{\w:\ \|\w\| \leq 10\epsilon} \wh F_1(\w) + \min_{\w:\ \|\w\| \leq 10\epsilon} R(\w) \\ &\geq  R(\w^*_0) - 10\epsilon, \numberthis \label{eq:rerm_fails_5}
\end{align*}
where the last inequality follows from the facts that $\wh F_1$ is 1-Lipschitz and $\wh F_1(0) = 0$. On the other hand, again using the $1$-Lipschitzness of $\wh F_1$, we have 
\begin{align*}
\wh F_1(\w^*_{\wh j}) &\leq \wh F_1(e_{\wh j}) + \nrm{ e_{\wh j} -  \w^*_{\wh j}} \\ 
&\leq -\frac{|S^-|}{n} + 10\epsilon \\
&\leq -\frac{1}{5} + 10\epsilon, \numberthis \label{eq:rerm_fails_6}
\end{align*}
where the inequality in the second line above follows from the definition of the special coordinate $\wh j$ and the point $\w^*_{\wh j}$. Combining \pref{eq:rerm_fails_5} and \pref{eq:rerm_fails_6} above and using the fact that $R(\w^*_{\wh j}) \leq R(\w^*_{j^*})$ 
(by definition of $j^*$), we get that
\begin{align*}
R(\w^*_{j^*}) -  R(\w^*_0) > \frac{1}{5}  - 20\epsilon \numberthis \label{eq:rerm_doesnt_work3} 
\end{align*} 

% \ascomment{Why not make it $2 \epsilon$ everywhere? I am confused about why different ranges?} 

\paragraph{Distribution-2:} Now, consider the scenario where we sample the dataset $S$ of size $n$ from the distribution $\cD_2 := \cD(\frac{1}{10}, \frac{1}{2}, e_{j^*})$. The assumed performance guarantee of RERM implies that, with probability at least $0.9$, RERM  algorithm on the dataset $S$ returns an $\epsilon$-suboptimal minimizer of the population loss $F_2(\w) = \En_{z \sim \cD_2} \brk*{f(\w, z)}$ under $\cD_2$. 
% In this case as well, with probability at least $0.9$, RERM on $S$ finds an $\epsilon$-suboptimal minimizer for the population loss $F_2$ under $\cD_2$.  
Furthermore, note that $\En_{z \sim \cD_2}[y \cdot x[j^*]] = \frac{1}{10}$ in this case, where the sample $z \equiv (x, y, \alpha)$. From an application of Hoeffding bound, if $n \geq 500$, then with probability at least $1-1/e > 0.6$, we have that $\frac{1}{n}\sum_{z \in S}yx[j^*]\leq \frac{1}{6}$. Taking a union bound, we get that with probability at least $0.5$, both the events happen (i.e. RERM finds an $\epsilon$-suboptimal solution, and $\frac{1}{n}\sum_{z \in S} yx[j^*]\leq \frac{1}{6}$). Henceforth we condition on the occurrence of this event. 

Next, note that any $\epsilon$-suboptimal point $w$ with respect to $F_2(\w)$ must satisfy \pref{eq:rerm_doesnt_work10}, which in this case corresponds to the condition that  $\|\w - e_{j^*}\| \leq 10\epsilon$, which implies that $\|\w\| \geq 1 - 10\epsilon$. This suggests that the point  $\w^*_0$ (defined in \pref{eq:w_jstar_defn}) cannot be an $\epsilon$-suboptimal minimizer of $F_2$ since $\|\w^*_0\| \leq 10\epsilon < 1 - 10\epsilon$.  Thus $\w^*_0$ can not be a minimizer of the regularized empirical risk (as all RERM solutions are $\epsilon$-suboptimal w.r.t. the population loss $F_2$). 

Next, note that Since any $\epsilon$-suboptimal minimizer $\w$ of $F_2$ must satisfy $\|\w - e_{j^*}\| \leq 10\epsilon$, which implies that $\|\w\| \geq 1 - 10\epsilon$, we conclude that $\w^*_0$ cannot be an $\epsilon$-suboptimal minimizer of $F_2$ since $\|\w^*_0\| \leq 10\epsilon < 1 - 10\epsilon$. Using $\wh F_2$ to denote the empirical loss on $S$, we get that
\begin{align*}
\wh F_2(\w^*_0) + R(\w^*_0) &> \min_{\w:\ \nrm*{\w - e_{j^*}} \leq 10\epsilon} \prn[\big]{R(\w) + \wh F_2(\w)} \\ &\geq \min_{\w:\ \nrm*{\w - e_{j^*}} \leq 10\epsilon} R(\w) + \min_{\w:\ \nrm*{\w - e_{j^*}} \leq 10\epsilon} \wh F_2(\w) \\ &\geq R(\w^*_{j^*}) - 10\epsilon.  \numberthis \label{eq:rerm_fails_7}
\end{align*}
where the last inequality follows from the facts that $\wh F_2$ is 1-Lipschitz and $\wh F_2(e_{j^*}) = 0$. As for the LHS, using the fact that $\nrm*{\w^*} \leq 10\epsilon$ and $\wh F_2$ is 1-Lipschitz, we have
\begin{align*}
\wh F_2(\w^*_0) &\leq F_2(0) + 10\epsilon \\ &= \frac{1}{n}\sum_{(x, y, \alpha) \in S}y\|e_{j^*} \odot x\| + 10\epsilon \\ &= \frac{1}{n}\sum_{(x, y, \alpha) \in S}yx[j^*]+ 10\epsilon \leq \frac{1}{6} + 10\epsilon. \numberthis \label{eq:rerm_fails_8}
\end{align*}
Combining \pref{eq:rerm_fails_7} and \pref{eq:rerm_fails_8} above, we get  
\begin{align*}
    R(\w^*_{j^*}) - R(\w^*_0) \leq \frac{1}{6} + 20\epsilon. \numberthis \label{eq:rerm_doesnt_work4} 
\end{align*} 

\paragraph{Final Step:} Considering \pref{eq:rerm_doesnt_work3}  and \pref{eq:rerm_doesnt_work4} together, we get that $\epsilon > \frac{1}{1200}$, as required. 
\end{proof}

The proof of \pref{prop:nn} is given in \pref{app:NN_representations}. 

\clearpage 

==> files/temp_files/app_chaining.tex <==
%!TEX root=../paper.tex
\renewcommand{\ind}[1]{^{(#1)}} 
\section{Multi-pass SGD}
\label{app:multi-pass SGD}

\subsection{Multi-pass SGD pseudocode}

\newcommand{\algcomment}[1]{/* {#1} */}
\begin{algorithm}[H] 
\caption{Multiple-epoch stochastic gradient descent} 
\begin{algorithmic}[1]
\REQUIRE Initial point: $w_0$, Dataset: $D = \crl*{z_i = (x_i, y_i)}_{i=1}^n$, step size: $\eta$, number of epochs: $k$. 
\STATE Initialize $t \leftarrow 0$, $w\ind{0} \leftarrow w_0$. 
% \STATE Define $D_1 = \crl*{z_i}_{i=1}^{n/2}$, and $D_2 = D \setminus D_1$. 
\STATE Define $D_1 \ldef{} \crl*{z_i}_{i=1}^{n/2}$. 
\STATE Define $\wh F_{2}(w) \ldef{}  \frac{2}{n} \sum_{t=n/2}^n f(w, z_i)$. 
\STATE Set $\wh w_0 = w_0$. 

\COMMENT{Run $k$ epochs of SGD using the dataset $D_1$}

\FOR {$s \in \crl{1, \ldots, k}$}
\FOR {$j \in \crl{1, \ldots, n/2}$} 
%\STATE Update the variable $w$
\STATE $w \ind{t + 1} \leftarrow w\ind{t} - \eta \grad f(w\ind{t}, z_j).$ 
\STATE $t \leftarrow t + 1$.
\ENDFOR 

\COMMENT{Compute average of iterates in this epoch}

\STATE Define $\wh w_s \ldef{} \frac{1}{n} \sum_{i=0}^{n-1} w\ind{t - i}.$ 
%
%\IF {$\wh F_2(\wh w_s) \geq \wh F_{2}(\wh w_{s-1})$}
%\STATE \textbf{return} $\wh w_s$. 
%\ENDIF 
\ENDFOR 
\STATE Define $\wh \cW = \crl*{\wh w_1, \ldots, \wh w_k}$. 
\STATE \textbf{return} $\wh w \ldef{} \argmin_{w \in \cW} \wh F_2(w)$. 
\end{algorithmic} 
\label{alg:multipass_sgd} 
\end{algorithm} 

\subsection{Proof of \pref{thm:multi_pass_succeeds}}  



In this section, we will provide a function $f: \bbR^d \mapsto \bbR$ such that taking multiple passes of SGD on $f$ \ascomment{Complete the description here!} 
\ascomment{Extend the example to work with NN approximations. A lot of moving parts are there, so we need to be careful on what we write. }

\ascomment{ Return average in the last epoch. Andrew Wilson's paper, average does better, thus we should not average in the beginning. For single pass SGD this is exactly what people do. Say that this is the last iterate convergence for GD.}  

\subsection{Problem Setup} \label{sec:chaining} 
In the following, we formally set up our learning problem. $k$ denotes the total number of epochs made by   SGD algorithm, $n$ denotes the total number of data points available for learning and $d$ denotes the problem dimension. 
\paragraph{Supporting functions.} We first define some atomic functions which will be composed together to get out main construction in this section.   

\ascomment{Give a one line description of each of these functions! If you have time, add a picture!} 
\begin{enumerate} 
\item \textbf{Wavelet unit:} For any $s \in [k]$, define the function $\Psi_s: \bbR^{d/2^s} \mapsto \bbR$ as 
\begin{align*} 
\Psi_s(w) &= \begin{cases} 
4 \cdot 2^s \nrm*{w} - 1 & \text{when ~} \frac{1}{4 \cdot 2^s} \leq \nrm*{w} \leq \frac{2}{4 \cdot 2^s} \\ 
3 - 4 \cdot 2^s \nrm*{w} & \text{when ~} \frac{2}{4 \cdot 2^s} \leq \nrm*{w} \leq \frac{3}{4 \cdot 2^s} \\ 
0 & \text{otherwise} \\%\nrm*{w} \leq \frac{1}{4\sqrt{k}} \text{~or} \nrm*{w} \geq \frac{1}{2 \sqrt{k}} \\  
\end{cases}. 
\end{align*}

\item \textbf{Ramp unit:} For any $s \in [k]$, define the function $\Phi_s: \bbR \mapsto \bbR$ as 
\begin{align*}
	\Phi_s(u) &= \begin{cases}
 0  & \text{when ~} u \leq \frac{12}{2^s} \\ 
 \frac{1}{2} \prn*{2^s u - 12} & \text{when ~}  \frac{12}{2^s} \leq u \leq \frac{14}{2^s} \\ 
 1 & \text{when ~} u \geq \frac{14}{2^s} 
 \end{cases}. 
\end{align*}


\item \textbf{Optimization unit:} For any $s \in [k]$, define the function $g_s:\bbR^{d/2^s} \times (\bbR^{d/2^s} \times \bbR) \mapsto \bbR$ as 
\begin{align*} 
g_s(w, (x, y)) &\ldef{}  \frac{y}{64 \cdot 2^s \cdot \sqrt{\log(n)}} \nrm{w \odot x} \Psi_s(w) + \frac{4}{2^s \sqrt{n}} \max\crl[\Big]{\nrm*{w}, \frac{1}{4 \cdot 2^s}} - \frac{8}{4^s \cdot \sqrt{n}}.  \numberthis \label{eq:g_definition_app} 
\end{align*} 

\item \textbf{Drift unit:} For any $s \in [k]$, define the function $h_s:\bbR \mapsto \bbR$ as 
\begin{align*} 
h_s(u) &\ldef{}  - \frac{2}{2^s \cdot \sqrt{n}} \min\crl[\Big]{u, \frac{16}{2^s}}. 
\end{align*} 

\item \textbf{Step size unit:} Define the function $\rho:\bbR \mapsto \bbR$ as  
\begin{align*}
\rho(u) &= \begin{cases}
	\frac{1}{\sqrt{n}} & \text{if~} u \leq \frac{-1}{2 \sqrt{n}} \\ 
 \frac{1}{2 \sqrt{n}} - u & \text{if~} \frac{-1}{2 \sqrt{n}} < u \leq \frac{1}{2 \sqrt{n}} \\ 
	0 & \text{if~} \frac{1}{2 \sqrt{n}} \leq u \leq \frac{9}{\sqrt{n}} \\ 
	u - \frac{9}{\sqrt{n}} & \text{if~} u \geq \frac{9}{\sqrt{n}} 
\end{cases}. 
\end{align*}
\end{enumerate}


\paragraph{Data sample.}  Each datapoint $z$ is given by a pair $(x, y)$ where $x \in \bbR^d$ and $y \in \bbR^k$. For any $s \in [k]$, we define $x_s \in \bbR^{\frac{d}{2^s}}$ to denote all the coordinate of $x$ from index $d - \frac{d}{2^{s-1}} + 1$ to $d - \frac{d}{2^s}$, i.e. $x_s = x[d - \frac{d}{2^{s-1}} + 1, d - \frac{d}{2^s}]$. Additionally, we define $w_{k+1}$ to denote all the coordinates of $w$ from index $d - \frac{d}{2^k} + 1$ to index $d$. Similarly, for any $s \in [k]$, we define $y_s \in \bbR$ to denote the $s$-th coordinate of $y$. 

\paragraph{Main stochastic function / $k$-length chain.} Our main construction in this section, denoted by $f$ and defined below, depends on $k$ and $n$. The function $f$ consists of two sets of trainable variables $w \in \bbR^d$ and $u \in \bbR^{k+1}$, and is parameterized by a data sample $z \in \bbR^{d + k + 1}$. 

The variable $w$ is further split into $k+ 1$ partitions $w_1, \ldots, w_{k + 1}$ such that the variable $w_1$ represents the first $\frac{d}{2}$ coordinates of $w$, the variable $w_2$ represents the next $\frac{d}{4}$ coordinates, and so on till $w_k$, and $w_{k+1}$ represents all the remaining $\frac{d}{2^k}$ coordinates. Specifically, for any $s \in [k]$,  the variable $w_s \in \bbR^{d/2^{s}}$ represents the coordinates of $w$ from index $d - \frac{d}{2^{s-1}} + 1$ to index $d - \frac{d}{2^s}$. The variable $w_{k+1}$ represents all the coordinates of $w$ from index $d - \frac{d}{2^k} + 1$ to index $d$. Similarly, the variable $u$ is also further split into $k$ partitions $u_1, \ldots, u_{k+1}$, where for any $s \in [k + 1]$, the variable $u_{k} \in \bbR$ represents the $s$-th coordinate of $u$. Using the variables $w_1, \ldots, w_k, w_{k+1}$ and $u_1, \ldots, u_k, u_{k+1}$, the function $f: \bbR^d \times \bbR^{k+1} \times \bbR^{d + k + 1}$ is defined as 
\begin{align*} 
f(w, u, z) &= \frac{39}{3 \sqrt{n}} + h_1(u_1) + g_1(w_1, z_1) + \sum_{s=1}^{k-1} \Phi_s(u_s)  \prn{h_{s+1}(u_{s+1}) + g_{s+1}(w_{s+1}, z_{s+1})} + \rho(u_{k+1}). 
\end{align*} 
For convenience, we also introduce a dummy variable $u_0 = 15$, and a function $\Phi_0(u) \equiv 1$, so that we can write $f$ more compactly as
\begin{align*} 
f(w, u, z) &= \frac{39}{3 \sqrt{n}} + \rho(u_{k+1}) + \sum_{s=0}^{k-1} \Phi_s(u_s)  \prn{h_{s+1}(u_{s+1}) + g_{s+1}(w_{s+1}, z_{s+1})}.  \numberthis \label{eq:chain_function}
\end{align*} 

The function $f$ is an example of \textbf{chain function}, where the variables $u_s$ and $w_s$ are interleaved with each other. \ascomment{Give a reference here!} We define the $s$-th link of the chain by the function $\Phi_s(u_s)  \prn{h_{s+1}(u_{s+1}) + g_{s+1}(w_{s+1}, z_{s+1})}$ (as above). Further, the function $\Phi_s(u_s)$ is constructed to represent a continuous approximation to the indicator function. This implies that the $s$-th link is visible to the learning algorithm only if $u_{s} > \frac{12}{2^s}$. 

\paragraph{Learning dataset.} The dataset $D = \crl{z\ind{i} = (x\ind{i}, y\ind{i})}_{i=1}^n$ is a collection of  $n$ samples, such that for every $i \in [n]$, $x\ind{i}$ is drawn independently from $\uniform(\crl{-1, 1}^d)$, and $y\ind{i}$ is drawn independently from $\uniform(\crl{-1, 1}^k)$. We denote the joint distribution over $(x, y)$ by $\cD$. 

\paragraph{Initialization.}  The initial value of $w$ by $w_0 \sim \cN(0, \frac{1}{\sqrt{d}} \bbI_d)$, where $\bbI_d$ denotes the $d \times d$ identity matrix. We initialize the variable $u$ such that $u_s\ind{0} = 0$ for all $s \in [k+1]$.  

\subsection{SGD can only learn at a rate of $\frac{1}{\sqrt{n}}$}  
\begin{theorem} 

\end{theorem}


\subsection{Multiple-epochs of SGD learns at a rate of $\frac{1}{n}$ with $\log(n)$ epochs} 
In this section, we give performance guarantees for multiple-epoch stochastic gradient descent algorithm given in \pref{alg:multipass_sgd}. In particular, we consider the function $f(w, u, z)$ where $z$ represents the data sample, and take $k$ passes over the dataset $D$ of $n$ data samples. 

\begin{algorithm}[H] 
\caption{Multiple-epoch stochastic gradient descent} 
\begin{algorithmic}[1]
\REQUIRE Dataset $D=\crl*{z_i = (x_i, y_i)}_{i=1}^n$. 
\STATE Set $\eta = \frac{8}{\sqrt{n}}, k=\ceil*{\log(n)}$.
\STATE Initialize $w\ind{0} \sim \gaussian(0, \frac{1}{\sqrt{d}} \bbI_d)$, where $\bbI_d$ denotes the $d \times d$ identity matrix. 
\STATE Initialize $u\ind{0} = 0$.  
\FOR {$t \in \crl{1, \ldots, kn}$}
\STATE Compute the index $j_t$ of the data sample to use as  $$j_t = t \mod(n) + 1.$$ %.  \hfill {Index in $D$ of the data sampled used for update.}
\STATE Update the variables $(w, u)$ using gradient of the function $f(w, u, z)$ at the data sample $z \ind{j_t}$, i.e. $$(w\ind{t +1}, u\ind{t+1}) \leftarrow (w\ind{t}, u\ind{t}) - \eta \cdot \partial f(w\ind{t}, u\ind{t}, z\ind{j_t}).$$
\ENDFOR 
\ascomment{Change the algorithm to include validation as in the main body!} 
\end{algorithmic} 
\label{alg:multipass_sgd_app} 
\end{algorithm} 

\begin{theorem} \ascomment{fill} 
	
\end{theorem} 
\begin{proof} Let us recall the notation before proceeding with the proof. At any time $t \geq 0$, and for any $s \in [k]$, we use the notation $w_s\ind{t}$ to denote the value of the variable $w_s$ after taking $t$ steps in \pref{alg:multipass_sgd}. Similarly, $u_s\ind{t}$ denotes the value of the variable $u_s$ after time $t$. Further, our dataset $D$ has $n$ samples, and for the update at time $t$ in \pref{alg:multipass_sgd}, we use the sample point with the index given by $j_t = t \mod(n) + 1$. In the following proof, we will analyze the values $\crl{w_s\ind{t}, u_s\ind{t}}_{s \in [k+1]}$ as we take multiple passes over the dataset. 

Using \pref{lem:chaining_initial_values}, we get that for all $s \in [k]$, the initial value of variable $w_s$ satisfies $\nrm{w_s\ind{0}} \leq \frac{2}{2^s}$. Further note that, for any $s \in [k + 1]$, the SGD update step at time $t$ corresponds to, 
\begin{align*} 
w_{s}\ind{t + 1} &= w_{s} \ind{t} - \eta \cdot \partial_{w_{s}} f(w\ind{t}, u\ind{t},  z_{j(t), s}), 
\end{align*}
and similarly, 
\begin{align*}
u_{s}\ind{t + 1} &= u_{s} \ind{t} - \eta \cdot \partial_{u_{s}} f(w\ind{t}, u\ind{t},  z_{j(t), s}), 
\end{align*} where the step size $\eta = \frac{8}{\sqrt{n}}$. 

We note the following properties of the training dynamics. These are formally proven in \pref{app:chaining_training_dynamics}. 
\begin{enumerate}
\item For any $s \in [k]$, the variable $w_s$ appears in the function $g_s(\cdot, w)$ only, which appears in the $k$-th link of the chain. 
%Thus, for any $z \in \cZ$,  
%\begin{align*}
%\partial_{w_s} f(w, u, z) = \Phi(u_{s-1}) \partial_{w_s} g_s(w_s, z_s). 
%\end{align*} 
By definition, the function $\Phi(u_{s-1}) = 0$ if $u_{s-1} \leq \frac{12}{2^s}$ and $\Phi(u_{s-1}) = 1$ if $u_{s - 1} \geq \frac{14}{2^s}$. Thus, the variable $w_s$ is updated by the SGD algorithm only if $u_{s - 1}\ind{t} \geq \frac{12}{2^s}$. % Furthermore, when $u_{s - 1}\ind{t} \geq \frac{14}{2^s}$, the variable $w_s$ is updated using the stochastic gradient $\partial g_s(w_s, z)$ and thus in this case, we can think of $w_s$ as being updated by running SGD on the loss function $g_s(\cdot, w_s)$. 

\item  For any $s \in [k]$, the variable $u_{s}$ appears through the function $h_{s}(\cdot)$ in the $s$-th link and through the function $\Phi_s(\cdot)$ in the $s +1$-th link of the chain. For any $z \in \cZ$, 
\begin{align*}
\partial_{u_s} f(w, u, z) = \Phi_{s-1}(u_{s-1}) h_s'(u_s) + \Phi'_s(u_s) \prn*{g_{s + 1}(w_{s + 1}, z_{s + 1} + h_{s + 1}(u_{s + 1}))},  
\end{align*} 
and thus the variable $u_s$ is updated only if $u_{s-1} \geq \frac{12}{2^{s-1}}$ or if $u_s \geq \frac{12}{2^s}$. 

\item The variable $w_{k+1}$ does not appear in the function $f(\cdot, \cdot, z)$ for any $z$ and is thus never updated. 

\item 
\end{enumerate} 

\end{proof} 

%\paragraph{Notation for the generated iterates} 
%\begin{enumerate}
%\item We assume that our data variables are: $w_1, w_2, \ldots, w_k$, and $u_1, u_2, \ldots, u_k$. 
%\item For any variable $u_{r}\ind{t, s}$ denotes the value of $u_r$ after taking the $t$-th step in the $s$-th epoch. 
%\item Data-set is denoted by $z_1, z_2, \ldots, z_{n}$, which further has $z_{1, 1}, z_{1, 2}, \ldots, z_{1, k}$. The data point $z_{i, j}$ has $x_{i, j}$ and $y_{i, j}$. Note that these are fixed and independent of the time step which we are looking at right now. In the $s$-th epoch, we will consider the data slice $z_{1:n, s}$. 
%\end{enumerate}
%
%\paragraph{Here are the parameters that we will choose:} 
%\begin{enumerate}
%\item Step size: $\eta = \frac{8}{\sqrt{n}}.$   \ascomment{The factor of $8$ is important here! Fixed step size!}  
%\item Assume that $k = \log(n)$.  
%\item Number of steps for learning: $\frac{n}{2}$. 
%\item Number of steps for convergence: $\frac{n}{4}$. 
%\item Initial value: $\frac{1}{2^s}$ for each of the weights. 
%\item Final value: $\frac{1}{4 \cdot 2^s}$ for each of the weights. 
%\end{enumerate}
%
%
%\begin{align*}
%	\numberthis \label{eq:sgd_update_rule} 
%\end{align*}


\subsection{Supporting technical results}  

\subsubsection{Basic function properties}
\begin{lemma} 
\label{lem:chaining_lipschitz_bounds}
For any $s \in [k]$, 
\begin{enumerate}
	\item the function $\Psi_s(w)$ is $4 \cdot 2^{s}$-Lipschitz. 
	\item the function $\Phi_s(u)$ is $\frac{2^s}{2}$-Lipschitz. 
	\item the stochastic function $g_s(w, z)$ is $\frac{1}{8 \cdot 2^s \cdot \sqrt{\log(n)}}$-Lipschitz in the variable $w$ for all $z \in \cZ$.  
\end{enumerate} 
\end{lemma}
\begin{proof} Parts-(1) and (2) follow directly from the definition of the functions $\Psi$ and $\Phi$. In the following, we prove Part-(3) i.e. an upper bound on the Lipschitz constant of the function $g_s(\cdot, z)$.

\paragraph{Proof of Part-(3).} We start by noting that $\partial g_s(w, z) = 0$ whenever $\nrm*{w} \leq \frac{1}{4 \cdot 2^s}$. When $\nrm*{w} \geq \frac{3}{4 \cdot 2^s}$, we have that $\Psi_s(w) = 0$ and thus, 
\begin{align*}
	\partial g_s(w, z) &= \frac{4}{2^s \cdot \sqrt{n}} \frac{w}{\nrm*{w}}.  
\end{align*}
In this case, $\nrm*{\partial g_s(w, z)} \leq 4/(2^s \cdot \sqrt{n})$. Finally, when $w$ is such that $\frac{1}{4 \cdot 2^s} \leq \nrm*{w} \leq \frac{3}{4 \cdot 2^s}$, we have  
\begin{align*} 
\partial g_s(w, z) &= \frac{y}{64 \cdot 2^s \cdot \sqrt{\log(n)}} \prn[\Big]{\frac{w \odot x}{ \nrm*{w \odot x}} \Psi_s(w) + \nrm*{w \odot x} \Psi'_s(w)}  + \frac{4}{2^s \cdot \sqrt{n}} \frac{w}{\nrm*{w}}.
\end{align*}
Using Triangle inequality, we get that 
\begin{align*}
\nrm*{\partial g_s(w, z) } &\leq \frac{1}{64 \cdot 2^s \cdot \sqrt{\log(n)}} \prn*{ \abs{\Psi_s(w)}  + \nrm*{w \odot x} \nrm{ \Psi'_s(w)}} + \frac{4}{2^s \cdot \sqrt{n}}  \\ 
&\leq \frac{1}{64 \cdot 2^s \cdot \sqrt{\log(n)}} \prn*{1 + \frac{3}{4 \cdot 2^s} \nrm{ \Psi'_s(w)}} + \frac{4}{2^s \cdot \sqrt{n}}  \\ 
&\leq \frac{4}{64 \cdot 2^s \cdot \sqrt{\log(n)}} + \frac{4}{ 2^s \cdot \sqrt{n}}, 
\end{align*} where the second line above follows from the fact that $\Psi_s(w) \leq 1$ for any $w$, and the fact that $\nrm*{w \odot x} \leq \nrm*{w}$ and that $\nrm*{w} \leq \frac{3}{4 \cdot 2^s}$ in this case. The inequality in the last line holds because the function $\Psi_s(w)$ is $4 \cdot 2^s$ -Lipschitz. Under the assumption that $n \geq 50000$, in all the three cases for the range of $\nrm{w}$ above, we get that 
\begin{align*}
\nrm*{\partial g_s(w, z)} \leq \frac{1}{8 \cdot 2^s \cdot \sqrt{\log(n)}}. 
\end{align*}
The above implies that $g_s(w, z)$ is $\frac{1}{8 \cdot 2^s \cdot \sqrt{\log(n)}}$-Lipschitz in the parameter $w$ for any $z \in \cZ$. 
\end{proof} 

\begin{lemma} \label{lem:population_loss_is_convex} For any $s \in [k]$, the population loss $G_s(w_s) \ldef{} \En_{z \sim \cD}\brk*{g_s(w_s, z_s)}$ is a convex function in the variable $w_s$ for the distribution $\cD$ given in \pref{sec:chaining}.  
\end{lemma} 
\begin{proof} Since $x$ and $y$ are independent to each other, we note that 
\begin{align*}
G_s(w_s) &=  \En_{(x, y) \sim \cD}\brk*{g_s(w_s, (x_s, y_s)} \\ 
		     &= \frac{\En[y_s]}{64 \cdot 2^s \cdot \sqrt{\log(n)}} \En[\nrm*{w_s \odot x_s}] \Psi_s(w_s) + \frac{4}{2^s \sqrt{n}} \max\crl[\Big]{\nrm*{w_s}, \frac{1}{4 \cdot 2^s}} - \frac{8}{4^s \cdot \sqrt{n}} \\
		     &=  \frac{4}{2^s \sqrt{n}} \max\crl[\Big]{\nrm*{w_s}, \frac{1}{4 \cdot 2^s}} - \frac{8}{4^s \cdot \sqrt{n}}, 
\end{align*} where the equality in the last line follows from the fact that $y_s \sim \uniform(\crl{-1, 1})$, and thus $\En \brk*{y_s} = 0$. The function on the right hand side in the above suggests that the population loss $G_s$ is a convex function in the variable $w_s$.  
\end{proof} 

\begin{lemma} 
\label{lem:chaining_initial_values} 
Let the initial value $w\ind{0}$ be drawn from $\cN(0, \frac{1}{\sqrt{d}} \bbI_d)$. 
\end{lemma} 
\begin{proof} 
\ascomment{Complete the proof of this initialization lemma} 
Fix any $s \in [k]$, we note that $w\ind{0}_s \in \bbR^{d/2^s}$. Furthermore, for every $j \in [d/2^s]$, the coordinate $w_s\ind{0}[j]$ is sampled independently from  $\cN(0, \frac{1}{\sqrt{d}})$. Further, 
\begin{align*}
\nrm{w_s\ind{0}}^2 &= \sum_{j=1}^{d/2^s} \abs{w_s\ind{0}[j]}^2.  
\end{align*}
Since $\crl{w_s\ind{0}[j]}$ are drawn independently from $\cN(0, \frac{1}{\sqrt{d}})$, using the multiplicative Chernoff bound from \pref{lem:chernoff_multiplicative}, we get that with probabillity at least $1 - \delta$, 
\begin{align*}
\sum_{j=1}^{d/2^s}  \abs{w_s\ind{0}[j]}^2 &\leq (1 + \sqrt{\frac{3 \cdot}{d} \log(2/\delta)}) \frac{d}{2^s} \En \brk{\abs{w_s\ind{0}[j]}^2}
\end{align*}
\end{proof}

\begin{lemma}[$w_s$ has bounded norm]  
\label{lem:chaining_g_w_bounded} 
Let $s \in [k]$. Suppose that $\gamma \leq \frac{8}{\sqrt{n}} \leq \frac{1}{2}$, and let $w_s \in \cW_s$ be such that $\nrm*{w_s} \leq \frac{2}{2^s}$. Let $w_s^+ \ldef{} w_s - \gamma \cdot \partial g_s(w_s, z)$ for an arbitrary data point $z \in \cZ$. Then, $\nrm*{w_s^+} \leq \frac{2}{2^s}$. 
\end{lemma}
\begin{proof} We prove the lemma via a case analysis: 
\begin{enumerate}[label=(\alph*)] 
\item \textbf{case1: $\mathbf{\nrm{w_s} \leq \frac{1}{2^s}}$.}  An application of Triangle inequality implies that 
\begin{align*}
		\nrm{w^+_s} \leq \nrm*{w_s} + \gamma \nrm{\partial g_s(w_s, z)}. 
\end{align*} 

Using \pref{lem:chaining_lipschitz_bounds} and the fact that $\gamma \leq \frac{1}{2}$ in the above bound, we get that 
\begin{align*}
\nrm{w^+} \leq \nrm*{w} + \gamma \cdot \frac{1}{8 \cdot 2^s \sqrt{\log(n)}} \leq \frac{2}{2^s}. 
\end{align*}

\item \textbf{case2: $\mathbf{\frac{1}{2^s} < \nrm{w_s} \leq \frac{2}{2^s}}$.} We note that 
\begin{align*}
	\nrm{w^+_s}^2 &= \nrm{w_s - \gamma \partial g_s(w_s, z)}^2 \\ 
			&= \nrm{w_s}^2 + \gamma^2 \nrm*{ \partial g_s(w_s, z) }^2 - 2 \gamma \tri{w_s, \gamma \partial g_s(w_s, z)} \\
			&= \nrm{w}^2 + \gamma^2 \frac{16}{4^s n} - 2 \gamma \cdot \frac{4}{2^s \sqrt{n} } \nrm*{w}, 
\end{align*}
where the last line follows by using the fact that $\partial g(w, z) = \frac{4}{2^s \sqrt{n}} \frac{w}{\nrm*{w}}$ whenever $\nrm*{w} \geq \frac{1}{2^s}$. Next, plugging in the fact that $\nrm*{w_s} \geq \frac{1}{2^s}$ in this case, we can further bound the above as 
\begin{align*}
	\nrm{w^+_s}^2 &\leq \nrm*{w_s}^2 + \gamma^2 \frac{16}{4^s n} - 2 \gamma \frac{4}{4^s \sqrt{n}}  \leq \nrm*{w_s}^2,  
\end{align*} where the inequality in the last line holds because $\gamma \leq \frac{1}{2}$. 
\end{enumerate} 
Thus, in either case, $\nrm*{w_s^+} \leq \frac{2}{2^s}$, completing the proof. 
\end{proof} 


\subsubsection{Properties of iterates produced by multi-pass SGD algorithm} \label{app:chaining_training_dynamics} 
In the following technical results, we consider the behavior of variables $u_s$ and $w_s$ for any $s \in [k]$ as we do multiple passes of SGD algorithm. 


\begin{lemma}[optimization of $w_s$]  
\label{lem:chaining_w_settles} For any $s$ in $\crl*{2, \ldots, k}$, let $t_0$ denote any time such that  $u_{s-1}\ind{t_0} \geq \frac{14}{2^{s-1}}$ and $\nrm{w_{s}\ind{t_0}} \leq \frac{2}{2^s}$. Suppose that we continue to update the variables $u_{s-1}$ and $w_{s}$ using multipass SGD algorithm given in \pref{alg:multipass_sgd} with a step size $\eta = \frac{8}{\sqrt{n}}$. Then, after $\frac{n}{2}$ update steps, with probability at least $1 - n^{-1/16}$,   
\begin{align*}
 	\nrm{w_s\ind{t_0 + \frac{n}{2}}} \leq \frac{1}{4 \cdot 2^{s}}. 
\end{align*}
\end{lemma} 
\begin{proof} 
%Without any loss of generality, in the following proof, we will assume that $t \leq \frac{n}{2}$ so that the epoch number $r_0$ will not change if we take additional $\frac{n}{2}$ steps using the SGD algorithm.  In the case that $t > \frac{n}{2}$, we will finish the epoch $r_0$ in $n - t$ steps of SGD and then take the rest of the $t - \frac{n}{2}$ steps in the epoch $r_0 + 1$. \ascomment{why can we do this ? Independence definition! Variable notation refinement} Suppose that we update $w_s$ using SGD algorithm on the function $f$ with the data sequence given by $\crl{z_t}_{t \geq t_0}$. 
We first note that that the SGD update for the parameter $w_{s}$ for any time $t$ is given by:
\begin{align*} 
w_{s}\ind{t + 1} &= w_{s} \ind{t} - \eta \cdot \partial_{w_{s}} f(w\ind{t}, u\ind{t},  z_{j(t), s}) \\
&= w_{s} \ind{t} - \eta \cdot \Phi(u_{s-1}) \cdot \partial_{w_s} g_s(w\ind{t}_s, z_{j(t), s}) 
\end{align*} 
where the function $g_{s}(w_s, z)$ is given in \pref{eq:g_definition_app} and the index $j(t)$ in the dataset is given by $j(t) = t \mod(n) + 1$. Using \pref{lem:chaining_u_large}, we get that $u_{s-1}\ind{t} \geq \frac{14}{2^{s-1}}$ for all $t \geq t_0$, and thus, $\Phi(u\ind{t}_{s-1}) = 1$ for all $t \geq t_0$. This implies that the above update for $w_s$ for any $t \geq t_0$ is given by 
\begin{align*}
w_{s}\ind{t + 1} &= 	w_{s} \ind{t} - \eta \cdot \partial_{w_s} g_s(w\ind{t}_s, z_{j(t), s}).  \numberthis \label{eq:sgd_works_1} 
\end{align*}
 
 Let $\crl{w\ind{t}_s}_{t \geq t_0}$ denote the sequence of iterates generated by the above update rule with the starting point given by $w_s\ind{t_0}$ at $t = t_0$. Suppose that there is no time $\tau \in [t_0 + 1, t_0 + \frac{n}{2}]$ such that $\nrm{w_s\ind{\tau}} \leq \frac{1}{4 \cdot 2^s}$. In the following, we will show that this leads to a contraction, hence proving our desired claim.  

We prove the desired contradiction by analyzing the iterates produced by SGD updates on a slightly different function $\wt g_s(w_s, z)$ defined as 
\begin{align*}
\wt g_{s}(w_s, z) \ldef{}  \begin{cases}
	g_s(w_s, z) & \text{if}~ \nrm{w_s} \geq \frac{1}{4 \cdot 2^s} \\ 
	\frac{4}{2^s \sqrt{n}} \nrm{w_s} - \frac{8}{4^s \cdot \sqrt{n}} & \text{if}~ \nrm{w_s} \leq \frac{1}{4 \cdot 2^s} 
\end{cases},   \numberthis \label{eq:sgd_works_0} % \frac{y}{64 \cdot 2^s \cdot \sqrt{\log(n)}} \nrm*{w \odot x} \Psi_s(w) + \frac{4}{2^s \sqrt{n}}\nrm*{w} - \frac{8}{4^s \cdot \sqrt{n}}. 
\end{align*}
and let 
\begin{align*}
\wt G_s(\wt w_s) \ldef{} \En_{z \sim \cD} \brk*{\wt g_s(\wt w_s, z)} = \frac{4}{2^s \sqrt{n}} \nrm{w_s} - \frac{8}{4^s \sqrt{n}}.\numberthis \label{eq:sgd_works_5}
\end{align*}

Note that $\wt G_s(w_s)$ is convex in $w_s$ and that $\wt g_s(w_s, z)$  is $(8 \cdot 2^s \cdot \sqrt{\log(n)})^{-1}$-Lipschitz in the parameter $w_s$ for any $z \in \cZ$ (the proof follows similar to the proof of \pref{lem:chaining_lipschitz_bounds}-3). Further, let $\crl{\wt w\ind{t}_s}_{t \geq t_0}$ denote the sequence of iterates generated by running SGD algorithm on the function $\wt g_s(w_s, z)$, with the starting point $\wt w_s\ind{t_0} = w_s\ind{t_0}$ and using the following update rule  
\begin{align*}
\wt w_{s}\ind{t + 1} &= 	\wt w_{s} \ind{t} - \eta \cdot \partial_{\wt w_s} \wt g_s(\wt w\ind{t}_s, z_{j(t), s}).  \numberthis \label{eq:sgd_works_2}  
\end{align*} 

Note that $\nrm{\wt w_s\ind{t_0}} = \nrm{w_s\ind{t_0}} \leq 2/2^s$ and so by \pref{lem:chaining_g_w_bounded}, we have $\nrm{w_s\ind{t}} \leq  2/{2^s}$ for all $t \geq t_0$. Since $\wt G_s(w_s)$ is convex in $w_s$, invoking \pref{lem:SGD_gurantee_hp} with $\eta = \frac{8}{\sqrt{n}}$, $T = \frac{n}{2}$, $w_0 = \wt w_s\ind{t_0}$, $L = \frac{1}{8 \cdot 2^s \cdot \sqrt{\log(n)}}$, and $B = 2/{2^s}$ we get that with probability at least $1 - \delta$, 
\begin{align*} 
\frac{2}{n} \sum_{t=t_0 + 1}^{t_0 + \frac{n}{2}} \wt G_s(\wt w_s\ind{t}) - \wt G^*_s &\leq \frac{1}{16 \cdot 4^s \sqrt{n} \cdot \log(n)}  + \frac{1}{8 \sqrt{n}} \nrm{\wt w_s\ind{t_0} - \wt w^*_s}_2^2  + \frac{1}{2 \cdot 4^s \sqrt{n \log(n)}} \sqrt{4 \log\prn*{1/\delta}}.
\end{align*} 
From the definition of the function $\wt G_s$ in \pref{eq:sgd_works_5}, we note that $\wt w_s^* = 0$ and that $\wt G_s(\wt w_s^*) = -8/4^s\sqrt{n}$. Plugging this in the above bound and using the fact that $\nrm{\wt w_s\ind{t_0}} = \nrm{w_s\ind{t_0}} \leq 2/2^s$, we get that 
\begin{align*} 
\frac{2}{n} \sum_{t=t_0 + 1}^{t_0 + \frac{n}{2}} \wt G_s(\wt w_s\ind{t}) + \frac{8}{4^s \sqrt{n}} &\leq \frac{1}{16 \cdot 4^s \sqrt{n}}  + \frac{1}{2 \cdot 4^s \cdot \sqrt{n}}  + \frac{1}{2 \cdot 4^s \cdot \sqrt{\log(n)}} \sqrt{\frac{4 \log\prn*{1/\delta}}{n}}. \numberthis \label{eq:sgd_works_3}   
\end{align*}
% where $B = \max_{t~:~t - t_0 \leq \frac{n}{2}} \nrm{\wt w_s \ind{t}}$. 


Recall that we assumed that there is no time $\tau \in [t_0 + 1, t_0 + \frac{n}{2}]$ for which $\nrm{w_s\ind{\tau}} \leq 1/{4 \cdot 2^s}$. However, for any such $w$ for which $\nrm*{w} \geq 1/{4 \cdot 2^s}$, the functions $\wt g$ and $g_s$ are identical for every $z \in \cZ$ (by definition of $\wt g_s$ in \pref{eq:sgd_works_0}), i.e. $\wt g_s(w, z) = \wt g_s(w, z)$. Thus, the corresponding SGD updates are equal, and the iterates $\wt w_s\ind{t} = w_s\ind{t}$ for all $t' \in [t_0 + 1, t_0 + n/2]$. Plugging this in relation \pref{eq:sgd_works_3} and setting $\delta = n^{-1/16}$ we get that 
\begin{align*} 
\frac{2}{n} \sum_{t=t_0 + 1}^{t_0 + \frac{n}{2}} \wt G_s(w_s\ind{t}) + \frac{8}{4^s \sqrt{n}} &\leq \frac{1}{16 \cdot 4^s \sqrt{n}}  + \frac{1}{2 \cdot 4^s \cdot \sqrt{n}}  + \frac{1}{4 \cdot 4^s \cdot \sqrt{n}} \leq \frac{1}{4^2 \sqrt{n}}.    \numberthis \label{eq:sgd_works_4} 
\end{align*}
% where $B = \max_{t~:~t - t_0 \leq n/2} \nrm{w_s \ind{t}}$. An invocation of \pref{lem:chaining_g_w_bounded} implies that $\nrm{w_s\ind{t}} \leq  2/{2^s}$ for all $t \geq t_0$, and thus $B \leq 2/{2^s}$. 
% Using the bound on $B$ in \pref{eq:sgd_works_4}  and setting $\delta = \frac{1}{n^{1/16}}$, we get that with probability at least $1 - n^{-1/16}$, 
% \begin{align*} 
% \frac{2}{n} \sum_{t=t_0 + 1}^{t_0 + \frac{n}{2}} \wt G_s(w_s\ind{t})  &\leq \frac{1}{16 \cdot 4^s \sqrt{n}}  + \frac{1}{2 \cdot 4^s \sqrt{n}}  + \frac{1}{4 \cdot 4^s \sqrt{n} \cdot \log(n)} \sqrt{\log(n)} \leq \frac{1}{4^s \cdot \sqrt{n}}. 
% \end{align*} 
% Since, $\wt G_s(w) \geq 0$ for any $w$. 
The above implies that there exists a time $\tau \in [t_0 + 1, t_0 + \frac{n}{2}]$ such that 
\begin{align*}
\wt G(w_s\ind{\tau}) + \frac{8}{4^s \sqrt{n}} \leq \frac{1}{4^s \sqrt{n}}. 
\end{align*} 
Plugging in the value of $\wt G(w_s\ind{\tau})$ from \pref{eq:sgd_works_5} in the above relation, we get 
\begin{align*}
\frac{4}{2^s \sqrt{n}} \nrm{w_s\ind{\tau}} \leq \frac{1}{4^s \sqrt{n}}, 
\intertext{which further implies that }
 \nrm{w_s\ind{\tau}}  \leq \frac{1}{4 \cdot 2^s}. 
\end{align*}
The above contradicts the fact that there is no time $\tau \in [t_0 + 1, t_0 + \frac{n}{2}]$ such that $\nrm{w_s\ind{\tau}} \leq \frac{1}{4 \cdot 2^s}$, proving the desired claim. 

%
%We now prove our main claim by showing that that there exists a time $\tau \in [t_0, t_0 + \frac{n}{2}]$ such that $\nrm{w_s\ind{\tau}} \leq \frac{1}{4 \cdot 2^s}$. Assume that this is not the case, i.e. for all times $t' \in [t_0, t_0 + \frac{n}{2}]$, we have $\nrm{w_s\ind{t'}} \geq \frac{1}{4 \cdot 2^s}$. However, for any $w_s$ for which $\nrm{w_s} \geq \frac{1}{4 \cdot 2^s}$, we have that $g_s(w_s, z) = \wt g_s(w_s, z)$ for all $z \in \cZ$. Thus, the sequences of iterates $\crl{w_s\ind{t}}_{t \geq t_0}$ and $\crl{\wt w_s\ind{t}}$ are identical. Using \pref{lem:SGD_gurantee_hp} for the function $\wt g(\cdot, z)$,  with the initial point given by $\wt w_s\ind{t_0}$, step size $\eta = \frac{8}{\sqrt{n}}$ and setting  $T = \frac{n}{2}$, we get that with probability at least $1 - \delta$, 
%\begin{align*} 
%\frac{2}{n} \sum_{t=t_0}^{t_0 + \frac{n}{2} - 1} \prn*{ \wt G(w_s\ind{t}) - \wt G^*_s }  &\leq {\frac{\eta L^2}{2} + \frac{1}{2\eta T} \nrm*{w_s\ind{0} - w^*_s}_2^2}  + 2B L \sqrt{\frac{2 \log\prn*{1/\delta}}{T}}. 
%\end{align*}
%
%
%
%%Furthermore, the function $\wt g_s$ is identical to the function $g_s$ whenever $\nrm{w_s} \geq \frac{1}{4 \cdot 2^s}$. 
%%
%%
%%Let $\crl{\wt w\ind{t}_s}_{t \geq t_0}$ denote the sequence of iterates generated by running SGD algorithm, with the starting point as $w_s\ind{t_0}$, on the function $\wt g_s(w, z)$ where the data point $z$ is chosen from the sequence $\crl{z_{t}}_{t \geq t_0}$. Recall that $w_s\ind{t}$ denotes the corresponding sequence of iterated generated by running SGD algorithm $g_s(w, z)$ on the function 
%%
%%
%%
%%Thus, for any point $w_s$ for which $\nrm*{w_s} \geq \frac{1}{4 \cdot 2^s}$, running SGD 
%
%Since, $\nrm{w_s\ind{0}} \leq \frac{2}{2^s}$ and the step size $\eta = \frac{8}{\sqrt{n}} \leq \frac{1}{2}$, an application of  \pref{lem:chaining_g_w_bounded}  implies that for all $t \geq 0$, 
%\begin{align*}
%\nrm{w_s\ind{t}} \leq \frac{2}{2^s}.  
%\end{align*}
%
%We first note that for any $z \in \cZ$, the function $g(w, z)$ is $\frac{1}{8 \cdot 2^s \sqrt{\log(n)}}$-Lipschitz. Thus, an application of \pref{lem:SGD_gurantee_hp} implies that with probability at least $1 - \delta$, 
%\begin{align*} 
%\frac{1}{T} \sum_{t=1}^{T}\prn*{ F_w(w_s\ind{t}) - F_w^* }  &\leq {\frac{\eta L^2}{2} + \frac{1}{2\eta T} \nrm*{w_s\ind{0} - w^*_s}_2^2}  + 2B L \sqrt{\frac{2 \log\prn*{1/\delta}}{T}}. 
%\end{align*} 
%
%Setting $\eta = \frac{8}{\sqrt{n}}$, $T = \frac{n}{2}$, $B = \frac{2}{2^s}$, $L = \frac{1}{8 \cdot 2^s \cdot \log(k)}$ and $\delta = \frac{1}{n^{1/4}}$ in the above, we get that 
%\begin{align*}
%\frac{2}{n} \sum_{t=1}^{n/2} \prn*{ F_w(w_{t}) - F_w^* }  &\leq \frac{1}{16 \cdot 4^s \sqrt{n} \log^2(n)}  + \frac{1}{2 \cdot 4^s \sqrt{n} \log^2(n)} + \frac{1}{2 \cdot 4^s \sqrt{n}} \\
%&\leq \frac{1}{4^s \sqrt{n}}. 
%\end{align*}
%Thus, there exists a time $\tau$ which has the property that we desire. 	
\end{proof} 

\begin{lemma} 
\label{lem:w_s_unchanged}  For any $s \in [k]$, let $t_0$ denote any time such that $\nrm{w\ind{t_0}_s} \leq \frac{1}{4 \cdot 2^s}$. Then, for all times $t \geq t_0$, the iterate $w_s\ind{t}$ generated by SGD updates in \pref{alg:multipass_sgd} satisfies 
\begin{align*}
w_s\ind{t} = w_s \ind{t_0}, %\nrm{w\ind{t}_s} \leq \frac{1}{4 \cdot 2^s}. 
\end{align*}
and thus $\nrm{w_s\ind{t}} \leq \frac{1}{4 \cdot 2^s}$. 
\end{lemma}
\begin{proof} For any time $t \geq 0$, the SGD update for the parameter $w_{s}$ is given by:
\begin{align*} 
w_{s}\ind{t + 1} &= w_{s} \ind{t} - \eta \cdot \partial_{w_{s}} f(w\ind{t}, u\ind{t},  z_{j(t), s}) \\
&= w_{s} \ind{t} - \eta \cdot \Phi(u_{s-1}) \cdot \partial_{w_s} g_s(w\ind{t}_s, z_{j(t), s}) 
\end{align*} 
where the function $g_{s}(w_s, z)$ is given in \pref{eq:g_definition_app} and the index $j(t)$ in the dataset is given by $j(t) = t \mod(n) + 1$. However, note that $\partial_{w_s} g_s(w\ind{t}_s, z_{j(t), s}) = 0$ whenever $\nrm{w_s\ind{t}} \leq \frac{1}{4 \cdot 2^s}$. This implies that for all times $t \geq t_0$, 
\begin{align*}
w_s\ind{t + 1} = w_s\ind{t} = \cdots = w_s\ind{t_0}. 
\end{align*}
\end{proof} 

\begin{lemma}[Deterministic growth for $u_s$] 
\label{lem:chaining_u_deterministic_growth} 
For any $s \in [k]$, let $t_0$ denote any time such that  $u\ind{t_0}_{s-1} \geq \frac{15}{2^{s-1}}$ and $u_s \ind{t_0} \leq \frac{3.5}{2^{s}}$. Suppose that we continue to update the variables $u_{s-1}$ and $u_{s}$ using multipass SGD algorithm given in \pref{alg:multipass_sgd}. Then, we must take at least $\frac{8.5n}{16}$ update steps so that the variable $u_s$ satisfies
\begin{align*} 
u_s \geq \frac{12}{2^s}. 
\end{align*} 
\end{lemma} 
\begin{proof} For any time $t \geq 0$, the SGD update for the parameter $u_{s}$ is given by:
\begin{align*} 
	u_s\ind{t + 1}  &= u_s\ind{t} - \eta \cdot \partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t})
\end{align*} where the subgradient  $\partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t})$ is given by
\begin{align*}
	\partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t}) &= \Phi_{s-1}(u\ind{t}_{s-1}) h_{s}'(u\ind{t}_{s}) + \Phi_s'(u\ind{t}_{s}) \prn*{ g_s(w\ind{t}_{s + 1}, z_t) + h_{s+1}(u\ind{t}_{s + 1})}.
\end{align*} 
% \ascomment{Put subscripts in the variables $g$ and $h$ above and in all other proofs in this section.}
Further, when $u_{s}\ind{t} \leq \frac{12}{2^{s}}$ the function $\Phi_s(u_{s}\ind{t}) = 0$ and $\Phi_s'(u_{s}\ind{t}) = 0$ (by definition). Similarly, when $u_{s-1}\ind{t} \geq \frac{15}{2^{s-1}}$, the function $\Phi_{s-1}(u_{s-1}\ind{t}) = 1$. Thus, in this case, the SGD update step is given by,
\begin{align*}
u_s\ind{t + 1}  &= u_s\ind{t} - \eta \cdot h_{s}'(u\ind{t}_{s }) \\
						&=  u_s\ind{t} + \frac{2 \eta}{2^{s} \sqrt{n}}, 
\end{align*} where the equality in the second line holds by plugging in the value of $h_{s}'(u_s\ind{t})$ for $u_s\ind{t} < \frac{16}{2^{s}}$. Setting the value of $\eta = \frac{8}{\sqrt{n}}$ in the above, we get that, 
\begin{align*}
u_s\ind{t + 1}  &= u_s\ind{t} - \eta \cdot h_{s}'(u\ind{t}_{s }) \\
						&=  u_s\ind{t} + \frac{16}{2^{s} n}, 
\intertext{which further implies that for any $t \geq t_0$}
u_s\ind{t} &=  u_s\ind{t_0} + \frac{16 (t - t_0)}{2^{s} n}. 
\end{align*}

Since, $u_s\ind{t_0} \leq \frac{3.5}{2^s}$, the above implies that $t - t_0$ must be greater that $\frac{8.5}{16}n$ so that $u_s\ind{t} \geq \frac{12}{2^s}$. 
\end{proof} 

\begin{lemma}[$u_{s}$ does not grown too much when $u_{s-1}$ is on the ramp] 
\label{lem:loose_drift} 
For any $s \in [k]$, let $t_0$ denote any time such that  $u\ind{t_0}_{s-1} \geq \frac{12}{2^{s-1}}$ and $u_s \ind{t_0} \leq \frac{1}{\sqrt{n}}$. Suppose that we continue to update the variables $u_{s-1}$ and $u_{s}$ using multipass SGD algorithm given in \pref{alg:multipass_sgd}. Then, after $\frac{n}{5}$ update steps, the variable $u_s$ satisfies the bound
\begin{align*} 
u_s \leq \frac{3.5}{2^s}. 
\end{align*}
%Furthermore, $\abs{u_s}$ is  strictly non-decreasing for all $SGD$ updates after the $\frac{}{}$never decreases in all updates using SGD. 
\end{lemma} 
\begin{proof} For any time $t \geq 0$, the SGD update for the parameter $u_{s}$ is given by:
\begin{align*} 
	u_s\ind{t + 1}  &= u_s\ind{t} - \eta \cdot \partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t})
\end{align*} where the subgradient  $\partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t})$ is given by
\begin{align*}
	\partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t}) &= \Phi_{s-1}(u\ind{t}_{s-1}) h_{s}'(u\ind{t}_{s}) + \Phi_s'(u\ind{t}_{s}) \prn*{ g_s(w\ind{t}_{s + 1}, z_t) + h_{s+1}(u\ind{t}_{s + 1})}.
\end{align*} 
% \ascomment{Put subscripts in the variables $g$ and $h$ above and in all other proofs in this section.}
We now show inductively that for any $t \leq t_0 + \frac{n}{5}$, we have $u_{s}\ind{t} \leq \frac{1}{2^s} + \frac{16(t-t_0)}{2^sn}$. This is true for $t = t_0$ since $u_s\ind{t_0} \leq \frac{1}{\sqrt{n}} \leq \frac{1}{2^s}$. So assume it is true for some $t$ such that $t_0 \leq t \leq t_0 + \frac{n}{5}-1$. Then, we have $u_s\ind{t} \leq \frac{1}{2^s} + \frac{16(t-t_0)}{2^sn} \leq \frac{1}{2^s} + \frac{16}{5\cdot 2^s} < \frac{12}{2^s}$. Hence, $\Phi_s(u_{s}\ind{t}) = 0$ and $\Phi_s'(u_{s}\ind{t}) = 0$ (by definition). Thus, in this case, the SGD update step is given by,
\begin{align*}
u_s\ind{t + 1}  = u_s\ind{t} - \eta \cdot \Phi_{s-1}(u\ind{t}_{s-1}) h_{s}'(u\ind{t}_{s }) \leq u_s\ind{t} + \frac{16}{2^{s}n}, 
\end{align*} 
since $-h_s'(u) \leq -\frac{2}{2^{s} \sqrt{n}}$ for all $u$, $\Phi_{s-1}(u) \leq 1$ for all $u$, and $\eta = \frac{8}{\sqrt{n}}$. Hence, we have 
\[u_s\ind{t+1} \leq u_s\ind{t} + \frac{16}{2^{s}n} \leq \frac{1}{2^s} + \frac{16(t-t_0)}{2^sn} + \frac{16}{2^{s}n} = \frac{1}{2^s} + \frac{16(t+1-t_0)}{2^sn},\]
completing the induction. Finally, using the bound for $t = t_0 + \frac{n}{5}$, we have
\begin{align*} 
u_s\ind{t} &\leq \frac{1}{\sqrt{n}} + \frac{16}{5\cdot 2^{s}} \leq \frac{3.5}{2^s}. 
\end{align*} 
\end{proof} 

\begin{lemma}[Ramp climbing for $u_s$]   
	\label{lem:ramp_climbing} 
	For any $s \in [k]$, let $t_0$ denote any time such that $u\ind{t_0}_{s-1} \geq \frac{15}{2^{s-1}}$ and $u\ind{t_0}_{s} \geq \frac{12}{2^s}$. Suppose that we continue to update the variables $u_s$ using multipass SGD algorithm given in \pref{alg:multipass_sgd}. Then, with probability at least $1 - \frac{1}{n^2}$,   
\begin{align*} 
u_s\ind{t_0 + \frac{n}{5}} \geq \frac{15}{2^s}
\end{align*}
%Furthermore, $\abs{u_s}$ is  strictly non-decreasing for all $SGD$ updates after the $\frac{}{}$never decreases in all updates using SGD. 
\end{lemma} 
\begin{proof} 
Since $u\ind{t_0}_{s-1} \geq \frac{15}{2^{s-1}}$, by \pref{lem:chaining_u_large}, we conclude that $u\ind{t}_{s-1} \geq \frac{15}{2^{s-1}}$ for all $t \geq t_0$. Thus, for any $t \geq t_0$, the SGD update for the parameter $u_{s}$ is given by:
\begin{align*} 
	u_s\ind{t + 1}  &= u_s\ind{t} - \eta \cdot \partial_{u_s} f(u_s \ind{t}, w_s\ind{t}, z_{t})  \numberthis \label{eq:chaining_us_escapes1} 
\end{align*} 
where the subgradient  $\partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t})$ is given by
\begin{align*}
	\partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t}) &= \Phi_{s-1}(u\ind{t}_{s-1}) h_{s}'(u\ind{t}_{s}) + \Phi_s'(u\ind{t}_{s}) \prn*{ g_s(w\ind{t}_{s + 1}, z_t) + h_{s+1}(u\ind{t}_{s + 1})} \\
				&= - \frac{2}{2^s \sqrt{n}}  + \Phi'(u_s\ind{t}) \Big( \frac{y_t}{64 \cdot 2^{s+1} \log(n)} \nrm{w_{s+1}\ind{t} \odot x_{t}} \Psi(w_{s+1}\ind{t}) \\ 
				& \qquad \quad \qquad  + \frac{4}{2^{s+1} \cdot \sqrt{n}} \max\crl[\Big]{\nrm{w_{s+1}\ind{t}}, \frac{1}{4 \cdot 2^{s+1}}} - \frac{8}{4^{s+1} \sqrt{n}} + h_{s+1}(u_{s + 1}\ind{t}) \Big).  \numberthis \label{eq:chaining_us_escapes2}
\end{align*} 
The second equality above follows since $\Phi_{s-1}(u\ind{t}_{s-1}) = 1$ since $u\ind{t}_{s-1} \geq \frac{15}{2^{s-1}}$ for all $t \geq t_0$. Now define the random variable $M_t$ as 
\begin{align*} 
M_t = u_s\ind{t + 1} - u_s{\ind{t}}  - \frac{2 \eta}{2^s \sqrt{n}} +  \eta \cdot \Phi'(u_s\ind{t})\prn[\Big]{\frac{4}{2^{s+1}\sqrt{n}} \max \crl*{\nrm{w_{s+1}\ind{t}}, \frac{1}{4 \cdot 2^{s +1}}} - \frac{8}{4^{s+1} \sqrt{n}} + h(u_{s+1}\ind{t})}.    \numberthis \label{eq:chaining_us_escapes4}
\end{align*} 
From the update rule in \pref{eq:chaining_us_escapes1}, the value of subgradient from \pref{eq:chaining_us_escapes2} and by setting $\eta = \frac{8}{\sqrt{n}}$, we get that 
\begin{align*}
M_t = - \Phi'(u_s\ind{t}) \cdot \frac{y_t}{8 \sqrt{n} \cdot 2^{s +1} \cdot \log(n)} \nrm{w_{s + 1}\ind{t} \odot x} \Psi(w\ind{t}_{s + 1}). 
\end{align*}
We next note that $\crl*{M_t}_{t \geq t_0}$ is a martingale difference sequence as
\begin{align*}
\En \brk*{M_t \| w_{s + 1}\ind{t}, } &= - \Phi'(u_s\ind{t}) \cdot \frac{\En \brk*{y_t}}{8 \sqrt{n} \cdot 2^{s+1} \cdot \log(n)} \En_{x_t} \brk{\nrm{w_{s + 1}\ind{t} \odot x_t}} \Psi(w\ind{t}_{s + 1}) = 0, 
\end{align*}
where the last equality follows from the fact that $y_t$ and $x_t$ are independent of $w_{s+1}\ind{t}$ and $u_s\ind{t}$, $x_t$ is independent of $y_t$, and that $\En \brk*{y_t} = 0$. 
Furthermore, we also have that  
\begin{align*}
\abs*{M_t} &=  \abs[\Big]{\Phi'(u_s\ind{t}) \cdot \frac{\En \brk*{y_t}}{8 \sqrt{n} \cdot 2^{s+1} \cdot \log(n)} \En_{x_t} \brk{\nrm{w_{s + 1}\ind{t} \odot x_t}} \Psi(w\ind{t}_{s + 1})} \\ 
&\leq \frac{1}{32 \sqrt{n} \log(n)} \nrm{w_{s + 1}\ind{t}} \\ 
&\leq \frac{1}{16 \sqrt{n} \cdot 2^{s+1} \log(n)},  \numberthis \label{eq:chaining_us_escapes3} 
\end{align*}where the inequality in the second line holds because $\Psi(w_{s+1}\ind{t}) \leq 1$ (by definition) and because the function $\Phi(u)$ is $2^s/2$-Lipschitz, and that $y \in \crl{-1, 1}$. The last line holds due to \pref{lem:chaining_g_w_bounded} which implies that $\nrm{w_{s+1}\ind{t}} \leq 2/{2^{s+1}}$.  

Using Azuma's inequality (\pref{lem:azuma_inequality}) for the first $\frac{n}{5}$ terms in the martingale difference sequence $\crl{M_{t_0}}_{t \geq t_0}$, we get that with probability at least $1 - \delta$, 
\begin{align*}
\sum_{t=t_{0}}^{t_0 + n/5 - 1} M_t \geq -  \frac{1}{32 \sqrt{n} \cdot 2^s \sqrt{\log(n)}} \sqrt{\frac{n}{2} \ln(1/\delta)}. 
\end{align*} 
Setting $\delta = \frac{1}{n^2}$ in the above, we get, with probability at least $1 - \frac{1}{n^2}$, 
\begin{align*}
\sum_{t=t_{0}}^{t_0 + n/5 - 1} M_t \geq  - \frac{1}{32 \cdot 2^s}. \numberthis \label{eq:chaining_us_escapes4.5} 
\end{align*}
Next, the definition of $M_t$ in \pref{eq:chaining_us_escapes4} implies that 
\begin{align*}
	\sum_{t=t_{0}}^{t_0 + n/5 - 1} \!\!\!\!\! M_t &= u_s\ind{t_0 + \frac{n}{5}} - u_s\ind{t_0} - \frac{2 \eta}{2^s \sqrt{n}} \cdot \frac{n}{5} + \!\!\!\!\! \sum_{t=t_{0}}^{t_0 + n/5 - 1} \eta \Phi'(u_s\ind{t})\prn[\Big]{\frac{4}{2^{s+1}\sqrt{n}} \max \crl*{\nrm{w_{s+1}\ind{t}}, \frac{1}{4 \cdot 2^{s +1}}} - \frac{8}{4^{s+1} \sqrt{n}} + h(u_{s+1}\ind{t})} \\
	&\leq  u_s\ind{t_0 + \frac{n}{5}} - u_s\ind{t_0} - \frac{2 \eta}{2^{s} \sqrt{n}} \cdot \frac{n}{5}, \numberthis \label{eq:chaining_us_escapes5} 
\end{align*} where the last line follows by ignoring the last term which is always negative as $\nrm{w_{s+1}} \leq \frac{2}{2^{s+1}}$ due to \pref{lem:chaining_g_w_bounded}, and using the fact that $h_{s+1}(u_{s + 1}\ind{t}) \leq 0$. Comparing \pref{eq:chaining_us_escapes4.5}  and \pref{eq:chaining_us_escapes5}, using $\eta = \frac{8}{\sqrt{n}}$, we get that with probability at least $1 - \frac{1}{n^2}$, 
\begin{align*}
u_s\ind{t_0 + \frac{n}{4}} - u_s\ind{t_0} &\geq  \frac{2 \eta}{2^{s} \sqrt{n}} \cdot \frac{n}{5}  - \frac{1}{32 \cdot 2^s} = \frac{3.2}{2^{s}} - \frac{1}{32 \cdot 2^s} \geq \frac{3}{2^s}.
\end{align*} The above implies that with probability at least $1- \frac{1}{n^2}$, 
\begin{align*}
u_s\ind{t_0 + \frac{n}{4}}  &\geq u_s\ind{t_0} + \frac{3}{2^s} \geq \frac{12}{2^s} + \frac{3}{2^s} \geq \frac{15}{2^s}, 
\end{align*}
which proves the desired claim.  
\end{proof} 

\begin{lemma}
	\label{lem:chaining_u_large} For any $s \in [k]$, let $t_0$ denote any time such that  $u\ind{t_0}_{s} > \frac{14}{2^s}$. Then, $u_s\ind{t_0+1} \geq u_s\ind{t_0}$. Furthermore, if additionally $u\ind{t_0}_{s-1} > \frac{14}{2^{s-1}}$, then $u_s\ind{t_0 + \frac{n}{8}} \geq \frac{16}{2^s}$. 
\end{lemma}
\begin{proof} For any time $t \geq 0$, the SGD update for the parameter $u_{s}$ is given by:
\begin{align*} 
	u_s\ind{t + 1}  &= u_s\ind{t} - \eta \cdot \partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t})
\end{align*} where the subgradient  $\partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t})$ is given by
\begin{align*}
	\partial_{u_s} f(u\ind{t}, w\ind{t}, z_{t}) &= \Phi_{s-1}(u\ind{t}_{s-1}) h_{s}'(u\ind{t}_{s}) + \Phi_s'(u\ind{t}_{s}) \prn*{ g_s(w\ind{t}_{s + 1}, z_t) + h_{s+1}(u\ind{t}_{s + 1})}.
\end{align*}
Now, since $u_s\ind{t_0} > \frac{14}{2^s}$, we have $\Phi_s'(u_s\ind{t_0}) = 0$, by definition. Thus, the above SGD update rule is equal to 
\begin{align*}
	u_s\ind{t_0 + 1}  &= u_s\ind{t_0} - \eta \Phi_{s-1}(u\ind{t_0}_{s-1}) h_s'(u_s\ind{t_0}) \\ 
	&\geq u_s\ind{t_0},
\end{align*} 
since $\Phi_{s-1}(u\ind{t_0}_{s-1}) \geq 0$ and $h_s'(u_s\ind{t_0}) \leq 0$. This finishes the proof of the first part of the lemma.

For the second part, if additionally $u\ind{t_0}_{s-1} > \frac{14}{2^{s-1}}$, then by virtue of the proof of the first part, we have $u\ind{t}_{s-1} > \frac{14}{2^{s-1}}$ for all $t \geq t_0$, which implies that $\Phi_{s-1}(u\ind{t}_{s-1}) = 1$. Furthermore, as long as $u_s\ind{t} < \frac{16}{2^s}$, we have $h_s'(u_s\ind{t}) = \frac{2}{2^s\sqrt{n}}$. Thus for any $t \geq t_0$ such that $u_s\ind{t} < \frac{16}{2^s}$, the above SGD update rule becomes
\begin{align*}
	u_s\ind{t + 1}  &= u_s\ind{t} + \frac{2\eta}{2^s\sqrt{n}} = u_s\ind{t} + \frac{16}{2^sn}.
\end{align*} 
Since $u_s\ind{t_0} > \frac{14}{2^s}$, the above implies after $\frac{n}{8}$ update steps, we must have $u_s\ind{t_0 + \frac{n}{8}} \geq \frac{16}{2^s}$, as required.
\end{proof} 





==> files/temp_files/old_erm_proof.tex <==
\item We show that there exists an ERM algorithm fails to find $\epsilon$-suboptimal solution, in expectation, for any $\epsilon \leq 1/400$.  

In this proof, we will assume that $n \geq 100$. Assume, for the sake of contradiction, that the expected suboptimality gap for ERM is at most $\epsilon = 1/ 400$. Then, by Markov's inequality, with probability at least $0.9$ over the choice of sample set $S$, the suboptimality gap for ERM is at most $10\epsilon$. 

Suppose that the dataset $S = \crl*{z_i}_{i=1}^n$ is sampled i.i.d.\ from $\cD$ (given in \pref{eq:nn_distribution_defn}). The population loss $F(w)$ for the distribution $\cD$ is given by 
\begin{align*} 
   F(\w) &= \En_{z \sim \cD} \brk*{f(\w; z)} = \En_{x, y} \brk*{\abs{y - \relu (w_{2}^\top \relu \prn{\w_{1} \odot x})}}. \numberthis \label{eq:pop_loss_defn_nn} 
\end{align*} Noting that $y\sim \cB(1/4)$ and that $y$ is independent of $x$, we get that for any $w$, 
\begin{align*}
   F(\w) &= \frac{1}{4}\En_{x} \brk*{\abs{1 - \relu (w_{2}^\top \relu \prn{\w_{1} \odot x})}} + \frac{3}{4} \En_{x} \brk*{\abs{\relu (w_{2}^\top \relu \prn{\w_{1} \odot x})}} \\ 
   		    &\geq \frac{1}{4} + \frac{1}{2} \En_{x} \brk*{\abs{\relu (w_{2}^\top \relu \prn{\w_{1} \odot x})}},  \numberthis \label{eq:nn_inequality1} 
\end{align*} where the last inequality above follows from an application of the Triangle inequality. Now, consider any point $w' = (w'_1, w'_2)$ that is an $10\epsilon$-suboptimal solution for the population loss $F(w)$, i.e. 
\begin{align*}
F(w') - \min_{w} F(w) \leq 10 \epsilon.  
\end{align*} Since, $w^* = 0$ corresponds to a global minimizer for $F(w)$ (as shown in the proof of \pref{lem:f_linearizable}). Plugging in $\min F(w) = F(0) = \frac{1}{4}$ in the above and using the upper bound from \pref{eq:nn_inequality1} for $F(w')$, we get that 
\begin{align*} 
\En_{x} \brk*{\abs{\relu ({w'_{2}}^\top \relu \prn{\w'_{1} \odot x})}} \leq 20 \epsilon. 
\end{align*} Using the fact that $\relu(\tau) \geq 0$ for any $\tau$ and an application of Jensen's inequality in the above implies that 
\begin{align*} 
\relu ({w'_{2}}^\top \En_{x} \brk*{\relu \prn{\w'_{1} \odot x})} \leq 20 \epsilon. 
\end{align*} Since $x \sim \text{Uniform}(\crl{0, 1}^d)$, for any $j \in [d]$, we have $\En_{x} \brk*{\relu \prn{\w'_{1} \odot x})[j]} = \frac{1}{2} \cdot \relu(w)[j]$. Using this relation in the above bound gives us  
\begin{align*} 
\relu ({w'_{2}}^\top \En_{x} \brk*{\frac{1}{2} \relu \prn{\w'_{1}})} \leq 20 \epsilon, 
\intertext{which further implies that} 
\relu ({w'_{2}}^\top \En_{x} \brk*{\relu \prn{\w'_{1}}} \leq 40 \epsilon. \numberthis \label{eq:w_condition} 
\end{align*} We note that the condition in \pref{eq:w_condition}  must be satisfied by any $10\epsilon$-suboptimal solution $w'$. Furthermore, since $x \in \text{Uniform}(\crl*{0, 1}^d)$ and $y \sim \cB(1/4)$, due to symmetry, we only need to consider solutions where $w_2 \geq 0$. We define the set $\wt W$ as the set of all $w' = (w'_1, w'_2)$ such that $\relu ({w'_{2}}^\top \relu \prn{\w'_{1}}) \leq 40 \epsilon$ and $w_2' \geq 0$. 

Next, define the event $E$ such that all of the following hold: 
\begin{enumerate}[label=$(\alph*)$] 
\item $\sum_{i = 1}^n y_i \geq \frac{n}{8}$. 
\item There exists $\wh j$ such that $\wh j \neq j^*$ and $x[\wh j] = y_j$ for all $j \in [n]$.    
\item ERM using the dataset $S$ returns an $10\epsilon$-suboptimal solution for the test loss $F(w)$. 
\end{enumerate} 
Using Hoeffding's inequality and the facts that $\En[y] = 1/4$, we get that part (a) holds with probability at least $0.5$ for $n \geq 100$. Furthermore, by \pref{lem:datatset_properties_basic_sco}, part (b) holds with probability at least $0.9$, and part (c) holds with probability $0.9$ by our assumption. Hence, the event $E$ occurs with probability at least $0.3$. In the following, we condition on the occurrence of the event $E$. 

Now, consider the point $\wh w = \prn{e_{\wh j}, e_{\wh j}}$ where $\wh j$ is defined in the event $E$. Using the inequality \pref{eq:nn_inequality1}, and the fact that $F(w^*) = 1/4$, we get that   
\begin{align*} 
   F(\wh w) - F(w^*) &\geq \frac{1}{2} \En_{x} \brk*{\relu (e_{\wh j}^\top \relu  \prn{e_{\wh j} \odot x})} \\
   							  &= \frac{1}{2} \En_{x} \brk{x[\wh j]} = 0.25. 
\end{align*} Clearly, the point $\wh w$ is not an $\epsilon$-suboptimal solution for the population loss $F(w)$. Since we condition on the event that the ERM solution is $\epsilon$-suboptimal for the population loss $F$, the above implies that the point $F(\wh w)$ must not correspond to any ERM solution. However, in the event $E$, we have that the ERM solution is $40$-suboptimal and must thus belong to the set $\wt \cW$. Thus, we must have that 
\begin{align*}
\wh F(\wh w) &\geq \min_{{w \in \wt \cW }} \wh F(w).  \numberthis \label{eq:nn_inequality_2} 
\end{align*} For the left hand side, we have  
\begin{align*} 
\wh F(\wh w) &= \frac{1}{n} \sum_{i=1}^n f(\wh w; (x_i, y_i))  \\ 
					&= \frac{1}{n} \sum_{i=1}^n \abs*{y_i - \relu (e_{\wh j}^\top \relu  \prn{e_{\wh j} \odot x_i})} \\ 
					&=  \frac{1}{n} \sum_{i=1}^n \abs*{y_i - x_i[\wh j]}  \\  
					&= 0, \numberthis \label{eq:nn_inequality_3} 
\end{align*} where the equality in the last line follows from the definition of the coordinate $\wh j$ as the one for which $y_i = x_i [\wh j]$ for all $i \in [n]$. On the other hand, for the right hand side of \pref{eq:nn_inequality_2}, we note that 
\begin{align*} 
 \min_{{w \in \wt \cW }} \wh F(w) &=  \min_{{w \in \wt \cW }} \,  \frac{1}{n}  \sum_{i=1}^{n} \abs[\big]{y_i - \relu (w_2^\top \relu  \prn{w_1 \odot x_i})} \\ 
 &\geq \frac{1}{n} \sum_{i=1}^{n} \abs{y_i} + \min_{w \in \wt \cW}  \prn[\big]{- \relu (w_2^\top \relu  \prn{w_1 \odot x_i})} \\ 
 &\geq \frac{1}{8} + \min_{w \in \wt \cW} \prn[\big]{ - \relu (w_2^\top \relu  \prn{w_1})} \\
 &\geq \frac{1}{8} - 40 \epsilon,  \numberthis \label{eq:nn_inequality_4} 
\end{align*} where the inequality in the second line follows by an application of Triangle inequality, the third line follows by using the fact that $\sum_{i=1}^n y_i \geq n /8$ and because $w_2 \geq 0$ for $w = (w_1, w_2) \in \wt \cW$. The last line above follows by the definition of the set $\wt \cW$. 

\ascomment{I do not know how to lower bound this without saying that we can replace $x_1$ by $\mb{1}$ and then use the definition of $\wt \cW$ to get \pref{eq:nn_inequality_4}. We can not upper bound x by $\mb{1}$ unless we have that $w_2[j] > 0 $ for all $j \in [d]$.\\} 
Plugging in the bound \pref{eq:nn_inequality_3} and \pref{eq:nn_inequality_4} in \pref{eq:nn_inequality_2}, we get that 
\begin{align*}
40\epsilon &\geq \frac{1}{8},   
\end{align*} 
which implies that $\epsilon \geq 1 / 400$, a contradiction, as desired. 
\end{enumerate} 	

